Deep learning architectures for automated image segmentation

Image segmentation is widely used in a variety of computer vision tasks, such as object localization and recognition, boundary detection, and medical imaging. This thesis proposes deep learning architectures to improve automatic object localization and boundary delineation for salient object segmentation in natural images and for 2D medical image segmentation. First, we propose and evaluate a novel dilated dense encoder-decoder architecture with a custom dilated spatial pyramid pooling block to accurately localize and delineate boundaries for salient object segmentation. The dilation offers better spatial understanding and the dense connectivity preserves features learned at shallower levels of the network for better localization. Tested on three publicly available datasets, our architecture outperforms the state-of-the-art for one and is very competitive on the other two. Second, we propose and evaluate a custom 2D dilated dense UNet architecture for accurate lesion localization and segmentation in medical images. This architecture can be utilized as a stand-alone segmentation framework or used as a rich feature extracting backbone to aid other models in medical image segmentation. Our architecture outperforms all baseline models for accurate lesion localization and segmentation on a new dataset. We furthermore explore the main considerations that should be taken into account for 3D medical image segmentation, among them preprocessing techniques and specialized loss functions.

==> 2D_Seg_Med/2d_seg.tex <==
\chapter{2D Medical Image Segmentation}
%2d dense unet model

After working with natural image segmentation, this chapter explores a specific and significant use case of segmentation, namely 2D and 3D medical image segmentation. Medical images can come in both 2D and 3D, depending on the equipment used to take the original images. The main advantage of using a 2D data-set over a 3D data-set is that it is more memory efficient and 2D models are more lightweight than 3D models, in terms of the number of learned parameters. Therefore 2D models can learn at a faster pace for accurate automatic delineation of lesion boundaries. Since deep learning models require a sizable amount of data to generalize due to a large number of learned parameters, working with exclusively 3D data can be difficult. 3D data can be sliced into 2D segments to create a larger 2D data-set for models to learn. The following sections present a number of deep learning models for the task of 2D lesion segmentation in medical images. 

In the past, segmentation of medical images was often done by hand and was cumbersome, time consuming and often error-prone. Early segmentation methods allowed for less human interaction but still required a user to initialize contours. The main objective of this chapter is the is to discuss the implementation of a deep learning model for fully automatic delineation of lesion boundaries in medical images. Accurate automated segmentation frameworks can be of huge assistance in early stages of medical assessment and detection of further health issues. However, this is a challenging task due to a number of factors, such as the inability to use priors for lesion segmentation, and low contrast images making boundary detection difficult, among others. Figure \ref{fig:2D_seg_pics} shows some example images of brain, lung, and liver to demonstrate how challenging this segmentation task is. This chapter through the steps to develop a novel 2D dilated dense UNet architecture for brain and lung segmentation.

For this task, a custom data-set of MRI and CT scans is used to detect lesions in the brain and lung. This data-set was developed in collaboration with Stanford University. Since this was not a publicly released dataset, the baseline was the results from a basic UNet model, discussed in the next section. The final dilated dense UNet performed significantly better than the baseline, confirming the effectiveness of the architecture.


% \begin{figure}
%   \includegraphics[width=\linewidth]{Images/2d_seg_pics.png}
%   \caption[Examples of Brain, Lung, and Liver Segmentation.]{Examples of brain, lung, and liver (row order) images. (a) original image, (b) ground truth segmentation, (c) overlay of ground truth on original image.}
%   \label{fig:2D_seg_pics}
% \end{figure}

\begin{figure}
\centering
\begin{tikzpicture}
\node (A) {\includegraphics[width=\linewidth]{Images/2d_seg_pics.png}};
\path (A.south west) -- (A.south east) node[pos=.34, below] {(a)} node[pos=.52, below] {(b)} node[pos=.69, below] {(c)};
\end{tikzpicture}
\caption[Examples of Brain, Lung, and Liver Segmentation.]{Examples of brain, lung, and liver (row order) images. (a) original image, (b) ground truth segmentation, (c) overlay of ground truth on original image.}
  \label{fig:2D_seg_pics}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%% UNet %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{UNet}
\subsection{Background}
%A general segmentation architecture can be broadly thought of as an encoder network followed by a decoder network \cite{encoder-decoder-overview}:
%\begin{enumerate}
  %\item The encoder is usually is a classification network like VGG/ResNet followed by a decoder network.
 % \item The decoder projects the discriminative features (lower resolution) learned by the encoder onto the pixel space (higher resolution) to get a dense classification.
%\end{enumerate}

The UNet architecture was first introduced by \cite{ronneberger2015u} as a method to perform segmentation for medical images. The advantage of this architecture over other fully connected models is that it consists of a contracting path to capture context and a symmetric expanding path that enables precise localization and automatic boundary detection with fewer parameters than an feed-forward network. Therefore this model was successful on small medical image data-sets. The basic UNet architecture implementation can be visualized in figure \ref{fig:unet}

\begin{figure}
  \includegraphics[width=\linewidth]{Images/unet.png}
  \caption{Basic UNet Model}
  \label{fig:unet}
\end{figure}

\subsection {Implementation}

First, a basic UNet architecture was implemented as a baseline performance on the Stanford data-set. The encoder portion was implemented by incrementally increasing the number of feature maps by powers of two, from 64 filters to 1024 filters at the bottom of the "U". The bottom of the "U" is at the lowest resolution to capture intricate details regarding the lesion shapes. In the decoder portion we decrease the number of feature maps by powers of 2, from 1024 to 64. The final image is passed through a softmax layer to produce the final binary segmentation map.

\textbf{Convolution}:
Each convolutional layer in the proposed architecture consists of a learned kernel $W$, a batch normalization and a rectified linear unit ReLU unit $r(X) = max(0, X)$ and can be described in Equation \ref{eq:conv}:

\begin{equation}
\begin{split}
\label{eq:conv}
c(X, W, \gamma) = r(b((X * W)), \gamma)
\end{split}
\end{equation}

W is a learned kernel; batch normalization b(X,$\gamma$) transforms the mean of each channel to 0 and the variance to a learned per-channel scale parameter $\gamma$. The ReLU unit r(X) = max(0, X) induces non-linearity and assists in gradient propagation. One convolutional block consists of a series of $c(X, W, \gamma)$ layers, as demonstrated in Figure \ref{fig:unet}.

\subsection{Results and Analysis}

\begin{table}[]
\centering
\begin{tabular}{lcccr}
\hline
Organ & Modality & Model: UNet \\ \hline\hline
Brain   & MRI      & 0.5231      \\
Lung    & CT       & 0.6646      \\
\end{tabular}
\caption{Dice score for UNet Model on Brain and Lung Datasets}
\label{table:Unet}
\end{table}

Table \ref{table:Unet} shows the results of the UNet model. From the results, it is clear that the UNet architecture alone is not enough to perform accurate segmentation. This could be due to the fact that some lesions are so small that as the encoder zooms into certain regions of the image, spacial information is lost. This hiders the ability of the model to pick up nuanced lesion shapes. Therefore, in the next section, the model is expanded by replacing the basic convolutional blocks of the UNet with dense blocks, described in the following section.

%%%%%%%%%%%%%%%%%%%%%%%%%% DENSE UNet %%%%%%%%%%%%%%%%%%%%%

\section{Dense UNet}

In the next iteration of the model, the convolutional blocks are replaced with dense blocks, as described in \cite{DenseNet}. The advantage of utilizing dense blocks is that each dense block is fed information from all previous layers, as discussed in the previous chapter. Therefore, as the network moves into deeper layers, information learned from shallower layers are not lost. Dense blocks consist of bottleneck layers. To move from one dense block to the next in the network, transition layers are utilized. In the following section, the implementation of the bottleneck and transition layers are described in more detail.

\subsection {Implementation}

%dense Block
\textbf{Dense Blocks}:

\begin{figure}
  \includegraphics[width=\linewidth]{Images/denseBlock.png}
  \caption[Dense Block Module.]{Dense Block Module. k is the growth rate. Before every dense block there are k feature maps generated by the transition layer. Within the dense block, there are n intermediate layers (IL), each contributing k feature maps (green block). The total number of feature maps produced is k + (n $\times$ k), or, the sum of the input maps and k times number of Intermediate Layers.}
  \label{fig:denseBlock}
\end{figure}

% dense block figure
Unlike UNets, classic convolution blocks are replaced with a version of dense blocks. Figure \ref{fig:denseBlock} illustrates the implementation of the dense block module. Dense blocks take in all features learned from previous layers and feed it into subsequent layers via concatenation. Dense connectivity can be described using Equation \ref{eq:dense_conv}. 

\begin{equation}
\begin{split}
\label{eq:dense_conv}
X_{l}  = H_{l}([x_{0}, x_{1}, . . . , x_{l - 1}])
\end{split}
\end{equation}

H() can be considered a composite function of batch normalization, convolution and ReLU unit. $[x_{0}, x_{1}, . . . , x_{l−1}]$ represents the concatenation of  all feature map from layers 0 to $l-1$. This is a more memory efficient because the model is not learning redundant features by duplicating feature maps. Direct connections are implemented between feature maps learned at shallow levels to deeper levels. 

The number of feature maps that are generated by each dense block is dictated by a parameter called the growth rate. For any dense block, the number of feature maps is calculated using Equation \ref{eq:num_feature_maps}

\begin{equation}
\begin{split}
\label{eq:num_feature_maps}
f_{i} = k + (k \times n)
\end{split}
\end{equation}

$f_{i}$ is the number of feature maps for dense block $i$. $k$ is the growth rate and $n$ is the number of dense connections to be made in dense block $i$. A visual representation of the feature maps in one dense block can be seen in Figure \ref{fig:denseBlock}. Before every dense block there are k feature maps generated by the transition layer. The growth rate regulates how much new information each layer contributes to the global state. Within the dense block itself, there are n connections made, hence to get the total number of filters, we sum the two value. It was found that for smaller datasets, smaller values of k (16-20) suffice to learn nuances of the data without over fitting, but perform better than a standard UNet.\newline
%bottleneck layer
\textbf{Bottleneck Layer}:

The dense UNet model has a moderate number of  parameters despite concatenating many residuals together since each 3x3 convolution can be augmented with a bottleneck.

A layer of a dense block with a bottleneck is as follows:

\begin{enumerate}
  \item Batch Normalization
  \item 1x1 Convolution bottleneck producing: grow rate ∗ 4 feature maps.
  \item ReLU activation
  \item Batch Normalization
  \item 3x3 Convolution producing: grow rate feature maps.
  \item ReLU activation
\end{enumerate}
%Transition layer
\textbf{Transition Layer}:

Transition layers are the layers between dense blocks. They perform convolution and pooling operations. The transition layers consist of a batch normalization layer and a $1 \times 1$ convolutional layer followed by a $2 \times 2$ average pooling layer. The transition layer is required to reduce the size of the feature maps by half before moving to the next dense block. This is useful for model compactness.

A transition layer is as follows:

\begin{enumerate}
  \item Batch Normalization
  \item 1x1 Convolution
  \item ReLU activation
  \item Average Pooling
\end{enumerate}

%Add Dense UNet model here

\begin{figure}
  \includegraphics[width=\linewidth]{Images/dense.png}
  \caption[Dense UNet Model.]{Dense UNet Model. In this design, convolutional blocks from \ref{fig:unet} are replaced with dense block on the encoder side. Transition layers are added for model compactness. The new modifications to this model are highlighted in red in the key.}
  \label{fig:densunet}
\end{figure}

Figure \ref{fig:densunet} illustrates the full Dense UNet architecture. 

\subsection{Results and Analysis}

\begin{table}[]
\centering
\begin{tabular}{lcccr}
\hline
Organ & Modality & Model: Dense UNet \\ \hline\hline
Brain   & MRI      & 0.5839     \\
Lung    & CT       & 0.6723     \\
\end{tabular}
\caption{Dice score for Dense UNet Model on Brain and Lung Datasets}
\label{table:DenseUnet}
\end{table}

Table \ref{table:DenseUnet} shows the results of the Dense UNet Model. There are many advantages of using the dense block modules. Recent work shows that with deeper convolutional networks, prediction accuracy is increased by creating shorter connections to layers close to both the input and the output, so that information is not lost as the network reaches deeper layers. In the standard UNet, let's assume each convolutional block have L layers. This means there are only L connections (one between each layer ie output of one layer is input of next and the next layer does not have information about layers prior to its immediate neighbor.) In the case of dense blocks, if there are L layers, there are L*(L+1)/2 direct connections being fed into the next block (ie direct, shorter connections to the input and output). This is advantageous for several reasons. Because of these direct connections, the vanishing gradient problem is alleviated and gets stronger feature propagation so that deeper layers do not lose information learned early on in the network as the resolution decreases. This also helps with memory. With careful concatenation, deeper layers have access to feature maps of shallow layers with only one copy of these feature maps in memory, instead of copies. 

%%%%%%%%%%%%%%%%%%%%%%% Dilated Dense %%%%%%%%%%%%%%%%%%%%%%

\section{Dilated Dense UNet}
\subsection{Background}

Next, a 2D dilated dense UNet is implemented for predicting a binary segmentation of a medical image. This architecture is described in Figure \ref{fig:dilateddensunet}. First, traditional convolution blocks of a UNet are replaced with dense blocks. Second, an up convolution method with learnable parameters is utilized. Third, dilation is added at the bottom of the architecture for better spatial understanding.

As can be seen in Figure \ref{fig:dilateddensunet}, the structure is still similar to that of the UNet. However, there are key differences which allow this model to outperform the basic UNet, for the medical image segmentation task. Unlike feed-forward convolutional neural networks, in which each layer only gets the feature maps from the previous layer, every layer of the dilated dense UNet structure takes as input all the feature maps learned from all previous layers via dense blocks for maximal information gain per convolution. This results in a model that has an overall greater understanding from a data-set in which a model has limited examples to learn and generalize from. In the dense blocks, each layer takes what is already learned before as input, to prevent redundant learning. To increase spacial understanding, dilation is added to the convolutions to further increase receptive fields at reduced resolutions and understand where lesions are relative to other lesions during segmentation. The decoder portion employs a series of up-convolution and concatenation with high-resolution extracted features from the encoder in order to gain better localization. The dilated dense UNet was designed to allow lower level features to be extracted from 2D input images and passed to higher levels via dense connectivity for more robust image segmentation.

%In our model, the encoder portion increases the receptive field while decreasing the spatial resolution by a series of successive dense blocks in lieu of convolution and pooling operations. 

\subsection {Implementation}

\textbf{Upconvolution}:
In our model, a different method of upsampling is proposed on the decoder side, as opposed to the bi linear interpolation done by \cite{ronneberger2015u}. Transpose convolutions are implemented to upsample. This is done because this method has parameters that can be learned while training, as opposed to a fixed method of interpolating, as done in bi linear interpolation. This allows for an optimal upsampling policy.

\textbf{Dilation}:
Dilated convolutions utilize sparse convolution kernels with large receptive fields, spatial understanding and the advantage of few training parameters. Dilation is added to  the bottom of the architecture, as shown in Figure \ref{fig:dilateddensunet}. 

% Assume the last block is x. D(x,d) represents the batch norm-convolution-reLU with dilation d on input x. Then, the dilation will take place like in the Equation \ref{eq:dilate_concat}:

% \begin{equation}
% \begin{split}
% \label{eq:dilate_concat}
% Y = [D(x,2); D(x,4);D(x,8); D(x,12)]
% \end{split}
% \end{equation}

% [D();D()] represents concatenations.  
The last dense block at the end of the contracting path is fed into 4 convolutional layers with dilation 2,4,8,16, respectively. Once the the blocks go through the dilated convolutions, they are concatenated together to get wider spatial perspective at the end of the contracting path of the dilated dense UNet. This is only effective and necessary at the end of the contracting path because this area is the lowest resolution and can lose track of spacial understanding. Therefore expanding the spacial context with dilation before continuing on the expanding path is an efficient and effective method for better results.

\begin{figure}
  \includegraphics[width=\linewidth]{Images/dilatedDense.png}
  \caption[Dilated Dense UNet Model.]{Dilated Dense UNet Model. In this design, we add dilation to the bottom of the network. The new modifications to this model are highlighted in red in the key.}
  \label{fig:dilateddensunet}
\end{figure}

Figure \ref{fig:dilateddensunet} illustrates the full Dense UNet architecture. 

\subsection{Results and Analysis}

\begin{table}[]
\centering
\begin{tabular}{lcccr}
\hline
Organ & Modality & Model: Dilated Dense UNet \\ \hline\hline
Brain   & MRI      & 0.6093     \\
Lung    & CT       & 0.6978     \\
\end{tabular}
\caption{Dice score for Dilated Dense UNet Model on Brain and Lung Datasets}
\label{table:DenseDilatedUnet}
\end{table}

%%%%%%%% EDIT THIS AFTER WE ADD RESULTS AND FINAL IMAGE %%%%%%%%
Table \ref{table:DenseDilatedUnet} shows the results of the dilated dense UNet model. It is observed that the dilated dense UNet model performed the best, in comparison to the basic UNet and the Dense UNet.

The work presented in this section was the backbone CNN used for a full pipeline proposed in the IEEE TMI 2019 submission \cite{ieeetmi2019}. The full pipeline consisted of the presented dilated dense UNet, which localized and determined initial lesion boundaries and produces an initial segmentation map. This map is fed into two functions to generate two probability feature maps $\lambda_{1}$ and $\lambda_{2}$. DLAC then uses these inputs (initial binary map, and two probability feature maps) to produce a more fine grained boundary for more accurate segmentation results.

% \begin{figure*}
%   \includegraphics[width=\textwidth]{Images/2d_final.png}
%   \caption[Examples of Final Segmentation Outputs.]{Examples of final segmentation outputs. (a) Ground Truth (b) Dilated Dense UNet output (c) DLAC output}
%   \label{fig:2d_final}
% \end{figure*}

\begin{figure}
\centering
\begin{tikzpicture}
\node (A) {\includegraphics[width=\linewidth]{Images/2d_final.png}};
\path (A.south west) -- (A.south east) node[pos=.24, below] {(a)} node[pos=.51, below] {(b)} node[pos=.77, below] {(c)};
\end{tikzpicture}
\caption[Examples of Final Segmentation Outputs.]{Examples of final segmentation outputs. (a) Ground Truth (b) Dilated Dense UNet output (c) DLAC output}
  \label{fig:2d_final}
\end{figure}

Figure \ref{fig:2d_final} shows some examples of the final segmentation produced by the dilated dense UNet and dilated dense UNet + DLAC models, in comparison to the ground truth, on the Stanford data-set. As a backbone, the dilate dense UNet is observed to do an exceptional job to localize and determine an initial boundary on the lesions. The DLAC supports the model further to refine the boundaries. Figure \ref{fig:2d_final}(b) validates that the dense dilated UNet can also be used as an effective, automated and accurate stand alone architecture for lesion localization and segmentation, as well. Thus we show that our custom dilated dense encoder-decoder is an effective backbone for the task of lesion localization for brain and lung lesion segmentation.


\section{Loss Function and Evaluation Metrics}

We utilize the dice coefficient as the loss function. The loss function is defined in Eq \ref{eq: DiceLoss}.

\begin{equation}
\begin{split}
\label{eq: DiceLoss}
Loss = 1 - \frac{2 \times |X \cap Y|}{|X| + |Y|}
\end{split}
\end{equation}

X is the prediction matrix and Y our ground truth matrix. $|X|$ stands for the carnality of the set X and $\cap$ for the intersection between X and Y. Dice coefficient is a heavily cited method for evaluating segmentation on medical images. It is observed to perform exceptionally on problems in which there is heavy class imbalanced in the data-set. This is indeed the case for the task of lesion segmentation, as can be seen by Figure \ref{fig:2D_seg_pics}. In the case of brain and lung segmentation, because so lesions are very small, there is a clear "class imbalance" between the number of pixels in the background and foreground of the image. Hence, the dice loss was utilized in our models.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Pretrained Model Analysis %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Effects of Using Pretrained Models}

One issue with segmentation involving medical images, is the lack of large aggregate data-sets. The proposed models required 2D images with binary masks indicating the location of lesions as labels. The Stanford data-set was rather small to see the full potential of this model, initially. When the model was initially trained on this small data-set, nice learning trends were not observed. The model overfit rather quickly. It was hypothesized that this was the case because there were not enough examples to properly generalize the model. Therefore, we ran experiments with and without the use of pretrained models. The results are seen in Table \ref{table:pretrain}.

\begin{table}[t]
  \centering
  \begin{tabular}{lcccccccccr}
  \hline
    Organ        & UNet       & DUNet     & Dilated DUNet    & UNet (P)    & DUNet (P)    & Dilated DUNet (P) \\ \hline\hline
    Brain        &    0.5231  &    0.5839 &    0.6093         & 0.5873      & 0.6105       & 0.7541     \\
    Lung         &    0.6646  &    0.6723 &    0.6978         & 0.7137      & 0.7028       & 0.8231      \\
  \end{tabular}
  \caption{Model Evaluations. Dice values for each model is presented above. (P) indicates that the model utilized pretrained weights. DUNet indicates Dense UNet.}
  \label{table:pretrain}
\end{table}

Segmentation for medical images is a particularly difficult task because priors cannot be utilized for predicting the shapes of lesions, since each lesion is so unique. Analyzing the results from Table \ref{table:pretrain}, indicate that using a pretrained model is clearly an effective strategy to help the model learn with such a small data-set. Pretraining can be thought of as a kind of "prior" added to the model to assist in the learning process when training on the data-set of interest. The pretraining allowed the 2D dilated dense UNet model to segment lesions with a dice score of 82 percent for lung and 75 percent for brain.





==> 2D_Seg_Natural/2D_Seg.tex <==
\chapter{2D Natural Image Segmentation}

%2d dense unet model

Manual delineation of boundaries of interest in segmentation is an error-prone procedure that is cumbersome, time intensive, and prone to user variability. Deep learning methods automate delineation by having learned parameters detect boundaries for segmentation. This chapter discusses the implementation of a series of deep learning models to improve object delineation of boundaries in the task of salient object segmentation in natural images. \textit{Natural} images are defined as images of everyday "natural" objects.

Encoder-decoder architectures have proven to be very effective in
tasks such as semantic segmentation. However, this architecture is yet to be
heavily explored for the salient object detection task. Therefore, a custom dilated dense encoder-decoder with depth wise separable convolution and dilated spatial pyramid pooling is proposed in this chapter. This is a simple and effective method to assist in object localization and boundary detection with spatial understanding.

The custom encoder-decoder architecture, as depicted in
Figure~\ref{fig:pipeline_nat}, is tailored to estimate a
binary segmentation map with accurate object boundaries. In this architecture, the encoder increases the size of the receptive field while decreasing the spatial
resolution by a series of successive dense blocks, and the decoder
employs a series of transpose convolutions and concatenations via skip
connections with high-resolution extracted features from the encoder.

The novelty in our architecture is that we create a custom dilated spacial pyramid pooling (DSPP) block at the end of the encoder. The output of the encoder is fed into 4 parallel dilation channels and the results are concatenated before passing it to the decoder, as seen in Figure \ref{fig:pipeline_nat}b. Since there are various features in natural images, such as complex boundaries, scale and resolution, dilated spacial pyramid pooling blocks are utilized to restore the spacial information that may have been lost while reducing resolutions on the encoder side for more accurate boundary detection of the salient object. The next sections systematically go through a series of architectures before arriving at the implementation for the novel dilate dense encoder-decoder with dilated pyramid pooling. The final architecture is validated on three prominent publicly available data-sets used for the task of salient object detection, namely MSRA, ECSSD, and HKU.

\section{Data-sets}

\subsection{Overview}

For the task of salient object detection, three data-sets were used, namely, ECSSD ,MSRA and HKU-IS. Table \ref{table:dataset_stats} shows the breakdown of the data-sets.

\begin{table*}[t]
\centering
\vskip 0.15in
\begin{center}
\resizebox{\textwidth}{!}{\begin{tabular}{lcccccr}
\hline
Data-set & \# Samples Train & \# Samples Valid  & \# Samples Test & Total Data-set Size \\
\hline
\hline
ECSSD \cite{yan2013hierarchical}       & 900  & 50 & 100 & 1050\\
MSRA \cite{WangDRFI2017}               & 2700  & 300 & 1447 & 4447\\
HKU-IS \cite{DBLP:journals/corr/LiY16} & 2663  & 337 & 2000 & 5000\\
\end{tabular}}
\end{center}
\caption{MSRA, ECSSD, and HKU Data-Set Breakdowns.}
\vskip -0.1in
\label{table:dataset_stats}
\end{table*}

There were some notable differences in the data-sets. The MSRA data-set
is mainly a collection of single objects that are centered in the
image. The outlines of most ground truth maps are simple to moderately
complex boundaries. However, there are several images in which the
salient object detection would be difficult, even for a human. These cases
are mainly when objects are partially occluded making it difficult to
distinguish what object is supposed to be detected. The ECSSD and
HKU data-sets had many examples with high complexity boundaries.
Most images contain, not one, but multiple salient objects and the
object outlines in the ground truth images were more complex. These
complexities substantially affect the contour evolution. For this
reason, the dilated dense encoder-decoder was developed to encapsulate varying spatial
information and boundaries in the image to give a solid starting point
to be fed into our ACM layer. The test sets are the same as those in
\cite{hou2016deeply} for the MSRA and HKU data-sets.
Since there was no specified test set for ECSSD, therefore 90 percent of
the data as used for training, 5 percent for validation, and 10 percent for
testing.

\section{Basic Encoder Decoder}

\begin{figure*}
  \includegraphics[width=\textwidth]{Images/basic_ed.png}
  \caption[Basic Encoder-Decoder Model.]{Basic Encoder-Decoder Model. The basic encoder-decoder model and a classic convolution + batch norm block and the associated produced feature maps is depicted.}
  \label{fig:baisc_ed}
\end{figure*}

\subsection{Background}

A basic encode-decoder architecture, illustrated in Figure \ref{fig:baisc_ed}, is first explored for the task of salient object detection.

\subsection {Implementation}

In the encoder portion, the number of learned feature maps is incrementally increased by powers of two, from 64 filters to 1024 filters at the end of the encoder portion. The size of the image is decreased by half at each stage of the encoder. The end of the encoder is at the lowest resolution to capture intricate details regarding the object shapes. In the decoder portion, the number of feature maps are decreased by powers of two, from 1024 to 64. The image dimensions are restored to the input dimensions, by doubling at each stage. The last layer is passed through a sigmoid filter to produce the final binary segmentation prediction probability mask. 

\textbf{Preprocessing}:
For this task, the original input image sizes were 300 by 400. The input images were resized to 256 by 256. This was done because 256 was the best value to minimize distortion but still make the data uniform to feed into the network.

\textbf{Convolution}: 
This basic encoder-decoder architecture utilized depthwised separable convolution. Each depth wise separable convolutional layer in the proposed
architecture can be formulated as follows:
\begin{equation}
\label{eq:1st}
c_{separable}(X, W, \gamma) = r(b((X * W)), \gamma). 
\end{equation}
It consists of an input $X$, a learned kernel $W$, a batch normalization $b$, and a ReLU unit $r(X) = max(0, X)$.  Depth wise separable convolution is used because it is a powerful operation that reduces the computation cost and number of learned parameters while maintaining similar performance to classic convolutions. 
% Classic convolutions are factorized into depth wise
% spatial convolutions over individual channels and point wise convolutions, and combines the results of convolutions over all channels.
Depth wise separable convolution factorizes classic convolution into depth wise convolutions and point wise convolutions over individual channels. The results of the two convolutions over all
channels are then combined.

\subsection{Results and Analysis}

\begin{table}[]
\centering
\begin{tabular}{lcccr}
\hline
Data-set &  $F_{\beta}$ & MAE \\ \hline \hline
ECSSD   &  0.737     & 0.120    \\
MSRA    &  0.805     & 0.093    \\
HKU     &  0.804     & 0.079    \\
\end{tabular}
\caption{$F_{\beta}$ and MAE scores for basic encoder-decoder model on ECSSD, MSRA, and HKU data-sets.}
\label{table:encoder-decoder}
\end{table}

The goal of the CNN architectures developed in this chapter is to create an efficient, simple and effective backbone that does not require pretrained models or expansive computational resources. As shown in Table~\ref{table:encoder-decoder}, a basic encoder-decoder structure alone, has mediocre performance. Reasons for this could include that, as an image goes deeper into the encoder, the framework loses information learned directly from higher resolutions. As a result, the model is unable to predict accurate image boundaries. This was especially observed when an image had multiple objects with more complex boundaries. In the next section, dense block are added to the encoder portion to mitigate this issue.

%%%%%%%%%%%%%%%%%%%%%%% Dilated Dense %%%%%%%%%%%%%%%%%%%%%%

\section{Dilated Dense Encoder-Decoder}

\begin{figure*}
  \includegraphics[width=\textwidth]{Images/final_cnn_arch.png}
  \caption[Dilated Dense Encoder-Decoder with Dilated Spacial Pyramid Pooling.]{Dilated Dense Encoder-Decoder with Dilated Spacial Pyramid Pooling. Dilated Dense Encoder-Decoder with Dilated Spacial Pyramid Pooling (DSPP) Block is depicted. Inside the DSPP, the output of the encoder is fed into 4 parallel dilations to increase the receptive fields at different scales, depicted in blue text.}
  \label{fig:pipeline_nat}
\end{figure*}

\subsection{Background}

The main differences between the basic encoder-decoder implementation and the custom encoder-decoder discussed in this section, are as follows:
\begin{itemize}
    \item Implementing dense block units
    \item Implementing a custom dilated spacial pyramid pooling block
\end{itemize}

In the next iteration of the encoder-decoder architecture, shown in Figure \ref{fig:pipeline_nat}, the basic convolutional blocks are replaced with dense blocks, as described in \cite{DenseNet}, in addition to using depthwise separable convolutions. The advantage of utilizing dense blocks is that each dense block takes information from all previous layers as its input. Therefore, at deeper layers of the network, information learned at shallower layers is not lost. A custom dilated spacial pyramid pooling block is added at the end of the encoder for better spacial understanding, as illustrated in Figure \ref{fig:pipeline_nat}b.

In this dilated dense encoder-decoder architecture, the encoder portion increases the receptive field while decreasing the spatial resolution by a series of successive dense blocks instead of convolution and pooling operations in typical UNet architectures. The bottom of the dilated dense encoder-decoder consists of convolutions with dilation to increase the spatial resolution for better image understanding. The decoder portion employs a series of up-convolutions and concatenations with high-resolution extracted features from the encoder in order to gain better localization and boundary detection and delineation. The dilated dense encoder-decoder was designed to allow lower level features to be extracted from 2D input images and passed to higher levels via dense connectivity for more robust image segmentation. 

\subsection {Implementation}

In each dense block, depicted in Figure \ref{fig:pipeline_nat}a, a composite
function of depth wise separable convolution, batch normalization, and
ReLU, is applied to the concatenation of all the feature maps $[x_{0},
x_{1},\dots, x_{l−1}]$ from layers 0 to $l-1$. The number
of feature maps produced by each dense block is $k + n \times k$. Each layer in the dense block contributes k feature maps to the global state of the architecture and each block has n intermediate layers ($n \times k$ term). The k layers that are generated by the transition layer at the end of the dense block are also added (the $k$ term). It was observed that a moderately small growth rate of
$k = 12$ was sufficient to learn decent segmentation, allowing us to
increase the model's learning scope with dense blocks without making
the model extremely heavy with learnable parameters. The tradeoff between better learning via more parameters and
still keeping the model relatively lightweight, using a smaller value
of $k$ was a consideration during model tuning for fast convergence. One reason for the success of a smaller growth rate is that
each layer has information about all subsequent layers and has
knowledge of the global state \cite{DenseNet}.
$k$ regulates the amount of new information that gets added to the
global state at each layer. This means that any layer in the network
has information regarding the global state of the entire network. Thus
it is unnecessary to replicate this information layer-to-layer and a
small $k$ is sufficient.

\textbf{Dilated Spacial Pyramid Pooling}:
Dilated convolutions make use of sparse convolution kernels to represent functions with large receptive fields and spatial understanding and with the advantage of few training parameters. Dilation is added to the bottom of the encoder-decoder structure, as shown in Figure \ref{fig:pipeline_nat}b. Assume the last block of the encoder is $x$. $D(x,d)$ represents the combined batch norm-convolution-reLU function, with dilation d on input $x$. Then, the dilation will take place like in Eq \ref{eq:dilate_concat}:

\begin{equation}
\begin{split}
\label{eq:dilate_concat}
Y = [D(x,2); D(x,4);D(x,8); D(x,16)]
\end{split}
\end{equation}

$[D();D()]$ represents concatenations. The output of the encoder, $x$, is fed into 4 parallel convolutional layers, $D(x,d)$, with dilation 2,4,8,16, respectively. Once the the blocks go through function D, they are concatenated together to get wider receptive field and spatial perspective at the end of the encoder. This is only done at the bottom of the architecture because this is the section with the least resolution since it is the the “deepest” part of the network. This allows for an expanded spatial context before continuing on the decoder path. 


\subsection{Results and Analysis}

\begin{table}[]
\centering
\begin{tabular}{lcccr}
\hline
Data-set &  $F_{\beta}$ & MAE \\ \hline \hline
ECSSD   &  0.825     & 078    \\
MSRA    &  0.857     & 0.061    \\
HKU     &  0.845     & 0.087    \\
\end{tabular}
\caption{$F_{\beta}$ and MAE Score for Dilated Dense Encoder-Decoder on ECSSD, MSRA, and HKU data-sets}
\label{table:dense_dilated_unet}
\end{table}

%%%%%%%% ADD MORE TO THIS %%%%%%%%
Table \ref{table:dense_dilated_unet} shows the results of the dilated dense encoder-decoder model with dilated spacial pyramid pooling. It is observed that this architecture performed significantly better than a basic encoder-decoder architecture, shown in Table \ref{table:encoder-decoder}.

% We also compare the results of other architectures that perform salient object detection on these 3 data-sets and present the results in \ref{table:data-sets-perf}. 

% \begin{table*}[t]
% \centering
% \label{sample-table}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lccccccr}
% \hline
% Model & ECSSD ($F_{\beta}$) & ECSSD (MAE)  & MSRA ($F_{\beta}$) & MSRA (MAE) & HKU ($F_{\beta}$) & HKU (MAE) \\
% \hline
% \hline
% RC \cite{inproceedings}               & 0.741  & 0.187 & 0.817 & 0.138 & 0.726 & 0.165 \\
% MDF \cite{DBLP:journals/corr/LiY15}             & 0.833  & 0.108 & 0.885 & 0.104 & 0.860 & 0.129 \\
% DRFI  \cite{WangDRFI2017}           & 0.787  & 0.166 & 0.855 & 0.119 & 0.783 & 0.143 \\
% UNet \cite{ronneberger2015u}            &  0.737 & 0.120 & 0.805 & 0.093 & 0.804 & 0.079 \\
% Our CNN          &  0.825 & 0.078 & 0.857 & 0.061 & 0.845 & 0.087 \\
% Our CNN + ACL    & \textcolor{green}{0.918}  & 0.048 & \textcolor{red}{0.881} & 0.046 & \textcolor{red}{0.861} & 0.054  \\
% SOA \cite{hou2016deeply}             & \textcolor{red}{0.915}  & 0.052 & \textcolor{green}{0.927} & 0.028 & \textcolor{green}{0.913} & 0.039 
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \caption{Model Evaluations. $F_{\beta}$ and MAE values for each model
% are presented.}
% \label{table:data-sets-perf}
% \end{table*}


\begin{table}[ht]
    \centering

   \resizebox{\textwidth}{!}{ \begin{tabular}{lccccccr}
\hline
Model & ECSSD ($F_{\beta}$) & ECSSD (MAE)  & MSRA ($F_{\beta}$) & MSRA (MAE) & HKU ($F_{\beta}$) & HKU (MAE) \\
\hline
\hline
%RC \cite{inproceedings}               & 0.741  & 0.187 & 0.817 & 0.138 & 0.726 & 0.165 \\
%MDF \cite{DBLP:journals/corr/LiY15}             & 0.833  & 0.108 & 0.885 & 0.104 & 0.860 & 0.129 \\
%DRFI  \cite{WangDRFI2017}           & 0.787  & 0.166 & 0.855 & 0.119 & 0.783 & 0.143 \\
MC  \cite{zhao2015saliency}                                  & 0.822 & 0.107 & 0.872 & 0.062 & 0.781 & 0.098\\
MDF \cite{DBLP:journals/corr/LiY15}             & 0.833  & 0.108 & 0.885 & 0.104 & 0.860 & 0.129\\
ELD \cite{lee2016deep}                                & 0.865 & 0.981 & 0.914 & 0.042 & 0.844 & 0.071 \\
ED \cite{ronneberger2015u}            &  0.737 & 0.120 & 0.805 & 0.093 & 0.804 & 0.079 \\
DDED       &  0.825 & 0.078 & 0.857 & 0.061 & 0.845 & 0.087 \\
DDED + ACL    & 0.920  & 0.048 & 0.881 & 0.046 & 0.861 & 0.054  \\
SOA \cite{hou2016deeply}             & 0.915 & 0.052 & 0.927 & 0.028 & 0.913 & 0.039 
    \end{tabular}}
    \caption{Model Evaluations. $F_{\beta}$ and MAE values for each model on ECSSD, MSRA, and HKU data-sets. ED abbreviates encoder-decoder. DDED abbreviates dilated dense encoder-decoder. ACL abbreviates active contour layer.}
    \label{table:datasets-perf}
\end{table}

% \begin{table}[ht]
% \centering
% \resizebox{\textwidth}{!}{\begin{tabular}{rlrrrrrrr}
%   \hline
%  & X & MASHvstRap & MASHvsBEEML & tRapvsBEEML & frequency & Mash\_mean & BEEML\_mean & tRap\_mean \\ 
%   \hline
% 1 & ETS & 8.95e-04 & 7.35e-04 & 4.78e-06 &  10 & 0.52 & 0.67 & 0.30 \\ 
%   11 & ZnF\_C2H2 & 7.08e-21 & 2.09e-02 & 1.70e-26 &  54 & 0.55 & 0.64 & 0.25 \\ 
%   10 & Zn2Cys6 & 4.94e-04 & 5.50e-02 & 3.52e-06 &  17 & 0.38 & 0.61 & 0.13 \\ 
%   8 & IRF & 1.16e-06 & 6.65e-02 & 5.54e-08 &  10 & 0.52 & 0.62 & 0.28 \\ 
%   2 & FH & 1.27e-05 & 8.61e-02 & 5.20e-07 &  10 & 0.53 & 0.66 & 0.27 \\ 
%   3 & HLH & 2.49e-05 & 1.31e+00 & 4.27e-05 &  13 & 0.61 & 0.74 & 0.26 \\ 
%   4 & HMG & 8.73e-33 & 1.41e+00 & 3.49e-08 &  44 & 0.55 & 0.48 & 0.12 \\ 
%   12 & ZnF\_C4 & 2.92e-06 & 1.92e+00 & 1.03e-07 &  10 & 0.66 & 0.73 & 0.27 \\ 
%   9 & unknown & 3.15e-27 & 1.96e+00 & 5.38e-21 & 121 & 0.44 & 0.49 & 0.16 \\ 
%   5 & Homeo & 1.69e-164 & 6.26e+00 & 2.35e-75 & 158 & 0.72 & 0.73 & 0.17 \\ 
%   7 & Homeo, POU & 3.12e-12 & 7.36e+00 & 5.21e-12 &  11 & 0.69 & 0.70 & 0.18 \\ 
%   6 & Homeo  & 9.82e-13 & 9.73e+00 & 1.21e-05 &  19 & 0.67 & 0.65 & 0.14 \\ 
%   \hline
% \end{tabular}}
% \caption{Paired t-test of most common TF families for Pearson Correlations} 
% \end{table} 


The work presented in this section was used as the backbone CNN for a full pipeline proposed for an MDA 2019 submission, \cite{MDA2019}. The results are described in Table \ref{table:datasets-perf}. (ED) describes the results from a basic encoder-decoder, discussed in the previous section. (DDED) describes results from the stand alone dilated dense encoder-decoder, discussed in this section. The full pipeline consisted of the DDED backbone CNN and an active contour layer (ACL). The output of the dilated dense encoder-decoder is taken as input into the ACL, which then produces the final segmentation results, seen in (DDED + ACL). As observed in Table \ref{table:datasets-perf}, the DDED + ACL architecture beats the current state-of-the-art for the ECSSD data-set and is competitive with the state-of-the-art for the MSRA and HKU data-sets. The ECSSD data-set contained many images with highly complex boundaries. The full DDED + ACL framework accurately delineates object boundaries, resulting in an increased $F_{\beta}$ score for the ECSSD data-set. This demonstrates the strength of this framework, in which the backbone DDED was trained from random initialization but yielded competitive results, in comparison to other models (MC, MDF, ELD) that utilized pre-trained CNN backbones, such as ImageNet \cite{deng2009imagenet}, AlexNet \cite{krizhevsky2012imagenet}, GoogLeNet \cite{szegedy2015going} and OverFeat \cite{sermanet2013overfeat}. 

Figure \ref{fig:compare} illustrates the performance of the ED, DDED, and DDED + ACL frameworks for precise boundary delineation. The images are grouped into categories highlighting different characteristics of the images. The grouping is utilized to indicate the success of the DDED and the DDED + ACL frameworks in a variety of cases. It is observe that all of the images from the dilated dense encoder-decoder (e), are much closer to the ground truth (b) than the results from basic encoder-decoder (d). Therefore (e) is a very robust backbone architecture for this segmentation pipeline, which is required for accurate boundary detection of the ACL. The results in (d) also indicate that the dilated-dense encoder-decoder model can also be a successful stand alone model, as almost all images produced are very close to the ground truth (b). 

% \begin{figure*}
%   \includegraphics[width=\textwidth]{Images/compare.png}
%   \caption[Examples of Segmentation Outputs.]{Examples of Segmentation Outputs. The last column is the segmentation produced by the dilated dense encoder-decoder. (a) Original image. (b) Ground truth. (c) DDED + ACL output segmentation. (d) ED output segmentation. (e) DDED output segmentation. }
%   \label{fig:compare}
% \end{figure*}

\begin{figure*}[!h]
  \centering
  \begin{subfigure}{\textwidth}
  \\Simple Scene $|$ Center Bias\newline
    \includegraphics[width=0.7\textwidth]{Images/r1.png}
  \end{subfigure}
  
  \begin{subfigure}{\textwidth}
  \\ Large Object $|$ Complex Boundary\newline
    \includegraphics[width=0.7\textwidth]{Images/r2.png}
    %\caption{More coffee.}
  \end{subfigure}
  
  \begin{subfigure}{\textwidth}
  \\Low Contrast $|$ Complex Boundary\newline
    \includegraphics[width=0.7\textwidth]{Images/r3.png}
    
    %\caption{Coffee.}
  \end{subfigure}
  
  \begin{subfigure}{\textwidth}
  \\Large Object $|$ Complex Boundary $|$ Center Bias\newline
  \begin{tikzpicture}
  
    %\includegraphics[width=0.7\textwidth]{Images/set5.png}
    \node (A) {\includegraphics[width=0.7\textwidth]{Images/r4.png}};
\path (A.south west) -- (A.south east) node[pos=.1, below] {(a)} node[pos=.30, below] {(b)} node[pos=.50, below] {(c)} node[pos=.70, below] {(d)} node[pos=.89, below] {(e)}
    \end{tikzpicture}
  \end{subfigure}
  \caption[Examples of Segmentation Outputs.]{Examples of Segmentation Outputs. The last column is the segmentation produced by the dilated dense encoder-decoder. (a) Original image. (b) Ground truth. (c) DDED + ACL output segmentation. (d) ED output segmentation. (e) DDED output segmentation. }
  \label{fig:compare}
\end{figure*}

%In Figure \ref{fig:compare} the dilated dense encoder-decoder produces a better segmentation than the basic encoder-decoder for almost all cases.  Thus we show that our custom dilated dense encoder-decoder is an effective backbone for the task of salient object detection. 

%%%%%%% ADD FIGURE TO SHOW SEGMENTATION RESULTS %%%%%%%



\section{Loss Function} %%%% CHANGE THIS

The dice loss function is utilized for this architecture. The loss function is defined in Eq \ref{eq: DiceLoss1}.

\begin{equation}
\begin{split}
\label{eq: DiceLoss1}
Loss = 1 - \frac{2 \times |X \cap Y|}{|X| + |Y|}
\end{split}
\end{equation}

X is the prediction matrix and Y is the ground truth matrix. $|X|$ stands for the carnality of the set X and $\cap$ for the intersection between X and Y. Dice loss gives more weight to correctly classified pixels, as seen by the term ($2 \times|X \cap Y|$). Therefore this loss function was selected for this case.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Eval metrics/augmentation/pretraining %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Evaluation Metrics}

Three evaluation metrics are utilized to validate the model performances, namely $F_{\beta}$, ROC curves, and mean absolute error (MAE). 

\textbf{$F_{\beta}$ Metric}: $F_{\beta}$
score measures the similarities between labels and predictions, using
precision and recall values, as follows:
\begin{equation}
\label{eq:f_beta}
F_{\beta} = (1+\beta) \times \frac{precision\times recall}{\beta
\times precision + recall}
\end{equation}

Precision and recall are two metrics that help understand the success of a deep learning model. Precision or recall alone cannot capture the performance of salient object detection. Based on the nature of the data-sets being used to validate the model, weights, dictated by the $\beta$ value, will be assigned to precision and recall, accordingly. We use the harmonic weighted average of precision and recall. In the case if salient object detection, there isn't a need to give more importance to either precision or recall, since all three data-sets were rather balanced in terms of class representation. Therefore, we decided to set $\beta = 1$ to
give equal weights to both precision and recall values. The results of
these studies are presented in Table \ref{table:datasets-perf}.

% \begin{figure}[t!]
% \begin{center}
%   \includegraphics[width=\textwidth]{Images/roc.png}
%   \caption[ROC Performance Curves for Salient Object Detection.]{ROC curves showing the performance of each architecture on ECSSD, MSRA, and HKU data-set.}
%   \label{fig:ROCCurve}
%   \end{center}
% \end{figure}

\begin{figure}
\centering
\begin{tikzpicture}
\node (A) {\includegraphics[width=\linewidth]{Images/roc.png}};
\path (A.south west) -- (A.south east) node[pos=.18, below] {(a)} node[pos=.52, below] {(b)} node[pos=.83, below] {(c)};
\end{tikzpicture}
\caption[ROC Performance Curves for Salient Object Detection.]{ROC curves showing the performance of each architecture on ECSSD, MSRA, and HKU data-set.} 
  \label{fig:ROCCurve}
\end{figure}

\textbf{ROC Curves}: In addition to the $F_{\beta}$, the ROC
metric is utilized to further evaluate the overall performance boosts that dense blocks and dilated spacial pyramid pooling adds to the salient object detection task. The ROC curves are shown in
Figure \ref{fig:ROCCurve}. A set of ROC curves was created for each of the three
data-sets. Each ROC curve consists of the results from testing the
architectures listed in Table~\ref{table:datasets-perf}, namely, a
basic encoder-decoder (ED), the custom dilated dense encoder-decoder (DDED), and the custom dilated dense encoder-decoder + ACL architectures (DDED + ACL). From the
curve trends, it is evident that the dilated dense encoder-decoder + ACL model outperforms the
others due to its high ratio of true positive rate (TPR) to false
positive rate (FPR); i.e., a majority TP cases and few FP cases.
Although ROC curves show the boost in performance gained by using the ACL in our architecture for all three data-sets, it is observed that the stand alone dilated dense encoder-decoder architecture performs significantly well in comparison to the basic encoder-decoder model, indicating that it too can perform accurate object boundary delineation. This is observed especially in the ECSSD and MSRA data-set, in Figure \ref{fig:ROCCurve}, since the trends for DDED and DDED + ACL are very close. 

\textbf{Mean Absolute Error}: The mean absolute error metric calculates the amount of difference, or "error" between the prediction and the ground truth. We utilized the
MAE score for model evaluation, as follows:
\begin{equation}
\label{eq:f_beta}
MAE = \frac{1}{W\times H}\sum_{x=1}^{W}\sum_{y=1}^{H}S(x,y) - G(x,y).
\end{equation}
where $W$ and $H$ are the pixel width and height of the prediction
mask $S$, and $G$ is the ground truth mask, which is normalized to
values $[0,1]$ before the MAE is calculated.

\subsection{Data Augmentation and Pretraining}

% \begin{figure*}
%   \includegraphics[width=\textwidth]{Images/augment.png}
%   \caption[Examples of Augmentation.]{Examples of Augmentation. (a) is the original image, (b) left-right flip, (c) up-down flip, (d) 90 deg rotation, (e) 180 deg rotation, (f) 270 deg rotation, (g) 1.3 scale zoom, (h) 1.7 scale zoom, (i) 1.9 scale zoom.}
%   \label{fig:augment}
% \end{figure*}

\begin{figure*}
  \begin{tikzpicture}
    %\includegraphics[width=0.7\textwidth]{Images/set5.png}
    \node (A) {\includegraphics[width=\textwidth]{Images/augment.png}};
\path (A.south west) -- (A.south east) node[pos=.06, below] {(a)} node[pos=.17, below] {(b)} node[pos=.28, below] {(c)} node[pos=.39, below] {(d)} node[pos=.50, below] {(e)} node[pos=.61, below] {(f)} node[pos=0.72, below] {(g)} node[pos=.83, below] {(h)} node[pos=.94, below] {(i)};
    \end{tikzpicture}
    \caption[Examples of Augmentation.]{Examples of Augmentation. (a) is the original image, (b) left-right flip, (c) up-down flip, (d) 90 deg rotation, (e) 180 deg rotation, (f) 270 deg rotation, (g) 1.3 scale zoom, (h) 1.7 scale zoom, (i) 1.9 scale zoom.}
  \label{fig:augment}
\end{figure*}

Table \ref{table:dataset_stats} shows that the size of each data-set was considerably small but these data-sets were still utilize because they were publicly available and highly popular for the task of salient object detection. But the small size of the data-set did negatively affect initial attempts at training the models. As a result, The data-set was expanded by performing data augmentation on all three data-sets. Examples of the augmented data-set are shown in Figure \ref{fig:augment}. To augment the data, each image went under the following transformations:

\begin{enumerate}
  \item left-right flip
  \item up-down flip
  \item 90, 180, 270 degree rotations
  \item zooming on the image at 3 different scales
\end{enumerate}

% %add image of augmentation here

% Algorithm \ref{algorithm:augment} to augment the 3 data-sets:
% %%%%%%%%%%%%%%%%%%%%%% FIX %%%%%%%%%%%%%%%%%%%%%%%%%
% % \begin{algorithm}
% %  \For{\texttt{each dataset in [ECSSD, MSRA, HKU]}}
% %         \For{\texttt{each (image, label) pair in dataset}}
% %             \State \texttt{flip_left_right(image)}
% %             \State \texttt{flip_up_down(image)}
% %             \State \texttt{rotate_image(image, [90,180,270])}
% %             \State \texttt{zoom_image(image, [0.2, 0.5, 0.9])}
% %         \EndFor
% %  \EndFor
% %  \caption{Data Augmentation Algorithm}
% %  \label{algorithm:augment}
% % \end{algorithm}

% \begin{algorithm}
%  \For{\texttt{each dataset in [ECSSD, MSRA, HKU]}}
%         \STATE $X \leftarrow 1 / x$
%  \EndFor
%  \caption{Data Augmentation Algorithm}
%  \label{algorithm:augment}
% \end{algorithm}

With the augmentation, the size of each data-set grew by a factor of 8. However, training on each individual augmented data-set alone was still not enough to fully generalize the model. The data augmentation helped the ECSSD data-set, so the trained model from this step was used as a pretrained model for the MSRA data-set. Once the MSRA data-set was trained, this combined pretrained model was used to train on the HKU data-set. The HKU data-set was the most challenging due to more complex examples. Therefore the training was done in the order described. With this training approach, the models achieved the results presented in Table \ref{table:datasets-perf}. As can be seen, the DDED and DDED + ACL results are competetive with that of the current state-of-the-art for these data-sets. The state-of-the-art is claimed in \cite{hou2016deeply}. In this paper, the authors discuss utilizing VGGNet \cite{simonyan2014very} and ResNet-101 \cite{he2016deep} as their backbones. It is impressive that our custom dilated dense encoder-decoder backbone is competitive with that of the state-of-the-art without utilizing more sophisticated pretrained models. This demonstrates that our model is lightweight, efficient and highly accurate for more precise salient object detection.





==> 3D_Seg/3D_seg.tex <==
\chapter{3D Medical Image Segmentation}

In recent times, the rise of deep learning models for 2D medical image segmentation has been very prevalent and has seen much success. We have recently observed the same trend for 3D data. 
After discussing deep learning architectures for 2D medical image segmentation, we transition to exploring the considerations to take into account when developing deep learning architectures for 3D medical image segmentation. There are many advantages to 3D medical image data-sets. In addition to the information gained via 2D data-sets, 3D data-sets offer spacial coherence, which is quite beneficial for this task. Although 3D data is limited, it does provide important information that can help a deep learning model learn more accurate segmentation parameters. However, although 3D data provides a rich information we could not gain from 2D data, 3D data poses many challenges and transitioning to the 3D space is far from trivial. In this chapter, we present important considerations one should take into account when designing and implementing an efficient lightweight 3D medical image segmentation model. We then evaluate these considerations by testing a liver segmentation data-set on a 3D VNet architecture.

\section{Background and Data-set}

Organ segmentation of 3D CT scans is a challenging task because of the high shape and size variations of anatomy between different patients. Much like in the 2D case, discussed in Chapter 4, 3D medical images suffer from low contrast from surrounding tissue, making segmentation difficult.

In this this chapter, we focus on the task of liver segmentation in 3D CT Scans. In CT scans, the liver tissue is often difficult to identify because in the image, the intensity is similar to other organs around it, as can be seen in Figure \ref{fig:3d_liver}. This makes liver segmentation a very challenging problem. Automated segmentation is initially the first step in health evaluation, early disease detection and clinical treatment such as radiotherapy or computer assisted surgery. The ability to accurately isolate and segment the liver can be of incredible assistance in the clinical process. In this chapter, we utilize the liver data-set from the Medical Segmentation Decathlon (MSD) Challenge. For this task, given a 3D CT scan, we utilize a VNet to segment out the liver portion of the scan.

\section{3D-VNet}

%An interesting application for 3D image imaging is the segmentation of CT scans of the human neck and abdomen to detect swollen lymph nodes.  Lymph nodes are small structures within the human body that work to destroy harmful substances. They contain immune cells that can help fight infection by attacking and destroying germs that are carried in through the lymph fluid. Therefore the lymphatic system is essential to the healthy operation of the body. The presence of enlarged lymph nodes is a signal to the onset or progression of a malignant disease or infection, therefore accurate segmentation models is critical to catch life threatening diseases at an early stage and support further treatment options.
%The task of detecting and segmenting swollen lymph nodes in CT scans comes with a number of challenges. 
%One if the biggest challenges is in CT scans, the abdominal region exhibits exceptionally poor intensity and texture contrast among neighboring lymph nodes as well as the surrounding tissues, seen in Figure \ref{fig:3d_lymph}. 
%To add to the challenge, abdominal lymph nodes often appear in clusters, making it hard to distinguish individual swollen nodes. Another difficulty is that low image contrast makes boundary detection between lymph nodes extremely ambiguous and challenging \cite{nogues2016automatic}. 3D lymph node segmentation is just one example out of the of many challenging 3D segmentation problems. Other difficult tasks include cancerous region segmentation in the lung, liver or brain. 
%%%%%%%%%%%%%% ADD MORE USE CASES?%%%%%%%%%%%%%%%%%%%%

When extending a deep learning architecture from 2D to 3D, there are several key points to consider. The first is the preprocessing techniques to be used. This includes image orientation (since we are not working in the 3D space), normalization methods, and how to fix large 3D images into memory. Another important consideration that makes quite a bit of difference in performance for 3D segmentation is the loss function we wish to use for training. In the following sections, we will describe these considerations in more detail so that the 2D medical image segmentation work presented in chapter 4 can be extended to the 3D domain in the future.

%The following U-Net like 3D encoder-decoder architecture is presented to tackle this challenging yet clinically relevant issue by presenting an efficient light-weight deep learning architecture for 3D segmentation.

\begin{figure*}
  \includegraphics[width=\textwidth]{Images/3d_liver.png}
  \caption{(a) Examples of the top, side and front view of the original CT scan (b) Examples of the ground truth mask (red) overlaid on top of the CT scans. In the original image, the contrast is so low it is difficult to distinguish the liver segment even with the human eye.}
  \label{fig:3d_liver}
\end{figure*}
%REPHRASE https://arxiv.org/ftp/arxiv/papers/1812/1812.01049.pdf

\section{3D Data Preprocessing Techniques}

As mentioned above, segmentation in 3D does offer a rich variety of information, as opposed to 2D segmentation. However, 3D segmentation does come with a number of challenges, as listed below:

\begin{enumerate}
  \item One of the biggest challenges faced was the amount of memory we had to run our models. We had one 11GB Nvidia 1080x GPU and each raw image was 512 by 512 by 775. This was way too large to fit an entire image plus a simple 3D UNet.
  \item We face the issue of class imbalance, since within each sample, the background dominated the foreground. Therefore during training, the model was prone to overfit to the background class.
  \item Training time took much longer since there were more voxels (3D version of pixels) contributed to the calculation of the gradient and back propogation.
\end{enumerate}

We fed our data-set through the following pipeline in Figure \ref{fig:preprocess} to alleviate the issues listed above and properly preprocess the 3D data. In the next sections, we describe our preprocessing steps in more detail.

\begin{figure}
  \includegraphics[width=\linewidth]{Images/preprocess.png}
  \caption{Proprocessing Pipeline for 3D Data-set}
  \label{fig:preprocess}
\end{figure}

\subsection{Consistent Orientation Across Images}

Since we are working with 3D images, the idea of orientation becomes an issue of interest. Consistent orientation among all images is important to speed up training time. If there are multiple orientations, the network is forced to learn all orientation, and order to generalize, we will need more data, which is not easy to come by for 3D medical images. We use Nibable, which is an open source python library to read in medical images, determine 3D image orientation and reorient images, if required, We found that the orientation selection itself did not make a difference on training as long as the orientation was consistent throughout the data-set. 

\subsection{Normalization}

Normalization is a key step in the preprocessing pipeline for any deep learning task. Normalization is also very important for medical images and there are varying methods of doing this.The aim of normalization is to remove heavy variation in data that does not contribute to the prediction process and instead accentuate the features and differences that are of most importance. There are a few interesting methods that could be used specifically for medical image segmentation such as the following \cite{dltk_overview}:
\begin{enumerate}
  \item Voxel Intensity Normalization:   
  Voxel intensity Normalization is very dependent on the imaging modality. For images such as weighted brain MR images, a zero-mean unit variance normalization is standard procedure. This is done because the contrast in the image is usually set by an expert taking the MRIs and thus there is high variation in intensity based on user across image sets. This variation can be considered noise. Thus to get rid of this noise and standardize intensity across multiple intensity settings, we use a zero mean normalization. In contrast, CT imaging measures a physical quantity such as radio-density in CT imaging, where the intensities are comparable across different scanners. Therefore, for this modality, the standard normalization methodology is clipping or rescaling to a range such as [0,1] or [-1,1].
  
  \item Spacial Normalization:
   Normalizing for image orientation avoids the need for the model to learn all possible orientations of input images. This reduces both the need for a large amount of training data and training time. Since, as mentioned before, properly labeled medical data is often small in quantity, this is a very effective technique of normalization.  
\end{enumerate}

%FIX THIS
For our problem, we worked with 3D CT scans, so we employed both methods of normalization. In the first section, we discussed reorienting all images to match so that we reduce the need for large data-sets. We also perform voxel intensity normalization by rescaling all voxels in the images to a range of [-1,1] and the voxels in the labels to [0,1].

\subsection{Generating Segmentation Patches}

To tackle the issue of limited memory to work with, we explored the idea of generating segmentation patches. A single 3D image in the dataset was 512 by 512 by 775. With the memory constraints, using these raw images would only allow for a batch size of 1, which would result in an incredibly long training time, and very little flexibility to extend our deep learning architecture. Therefore, we adopted the idea of patch generation. 

The basic idea of patch generation is to take in an input image, determine the regions of most interest in the image, and return a smaller portion of the image, focusing on these regions of importance. Doing this is important for many reasons. The first reason is, having smaller image sizes allow for larger batch sizes and faster training The second reason is that the data is naturally augmented with this process. The third reason is that we can avoid the issue of class imbalance per image. Class imbalance occurs when a sample image has more voxels belonging to one class over another. Figure \ref{fig:3d_liver}b shows this very clearly. We see that in the example, the majority of the voxels belong to the background (black) class and a small subset belong to the foreground (red) class. Feeding such images directly to the model will cause the the model to skew  its learning to favor the background voxles. Therefore, intelligent selection of patches is key to training. For this work, we generated patches of 128 by 128 by 128. We utilized the Deep Learning Toolkit to generate our class balanced segmentation patches. %maybe expand more with diffferent patch selection techniques or explain the DLTK one

Unlike during training time, in which the patches are generated randomly around areas of interest, during test time, we systematically break the image into 128 by 128 by 128 chunks and predict the output on each option, and then join the predictions together to get our final prediction. Patching alone creates some discrepancies at the boarders of patches so we perform smoothing to get a more seamless prediction.

\section{3D VNet Implementation}

\subsection{Loss Functions and Evaluation Metrics}

For the VNet architecture, we decide to experiment with different loss functions to see how it affects the performance of the model. The choice of loss functions can significantly affect the performance of 3D segmentation architectures. We next discuss some loss functions in more detail to gain some intuition for why one would produce better results over another.

In medical images, it is very common that the region of interest,for example, a lesion or an organ, covers a very small portion of the scan. Therefore, during the learning process, the network often gets stuck in local minima due to this class imbalance of background and foreground pictures. This causes poor results during training and testing since the prediction of both classes is weighed equally. This causes the model to be biased toward the background voxels and the foreground is either completely missed or partially detected. The following losses attempt to address these issues.

% \begin{figure}
%   \includegraphics[width=\linewidth]{Images/preprocess.png}
%   \caption{Proprocessing Pipeline for 3D Data-set}
%   \label{fig:preprocess}
% \end{figure}

\paragraph{Jaccard Coefficient and Loss}

The Jaccard coefficient is measure of similarity between a ground truth mask and a prediction mask. Lets assume that all voxels in the ground truth mask are in set $G$. All voxels in the prediction mask are in set $P$. The Jaccard coefficient calculates the ratio of 3 mutually exclusive partitions: $|P \cap G|$, $|P \setminus G|$, $|P \setminus G|$. The equation for the Jaccard coefficinet is seen in eq \ref{eq: jaccard_c}.
\begin{equation}
\begin{split}
\label{eq: jaccard_c}
J = \frac{|P \cap G|}{|P \cap G| + |P \setminus G| + |P \setminus G|}
\end{split}
\end{equation}

The full loss function is defined as in eq \ref{eq: Jaccard_loss}.

\begin{equation}
\begin{split}
\label{eq: Jaccard_loss}
Loss = 1 - \frac{|P \cap G|}{|P \cap G| + |P \setminus G| + |P \setminus G|}
\end{split}
\end{equation}

The Jaccard coefficient calculates the overlap ratio between a ground truth mask and a predicted mask by giving equal weightage to  $|P \cap G|$, $|P \setminus G|$, $|P \setminus G|$. If the data one is working with does not suffer too much from class imbalance, the Jaccard coefficient and loss is a good metric to measure the success of a model. If there is class imbalance, this method may not produce as promising results and a model could become biased towards the dominating class. 

\paragraph{Dice Coefficient and Loss}

The Dice coeffient is another metric that compares the similarity between a ground truth mask and a prediction mask. It is similar to the Jaccard coefficient with one subtle but significant difference in the way class imbalance is handled. We utilized the Dice Loss in Chapter 4, as it is widely use loss function for both 2D and 3D medical image segmentation. The Dice coefficient, also known as the Sorensen-Dice coefficient, is defined as in eq \ref{eq: Dice_c}

\begin{equation}
\begin{split}
\label{eq: Dice_c}
D = \frac{2 \times |P \cap G|}{2 \times |P \cap G| + |P \setminus G| + |P \setminus G|}
\end{split}
\end{equation}

The full Dice Loss is as in eq \ref{eq: Dice_loss}. $|P \setminus G|$ notation refers to the set of elements in $P$ but not in $G$.

\begin{equation}
\begin{split}
\label{eq: Dice_loss}
Loss = 1 - \frac{2 \times |P \cap G|}{2 \times |P \cap G| + |P \setminus G| + |P \setminus G|}
\end{split}
\end{equation}

The Dice coefficient is a measure of similarity between two sets. The Dice Coefficient addresses the issue of class imbalance by calculating the overlap between a prediction and a ground truth mask for a region of interest. The Dice coefficient is unique because unlike the Jaccard metric, the Dice metric gives more weight to voxels that belong to both sets (aka the overlapping region of both sets) when calculating the overlap ratios, hence the factor of 2 that is multiplied to the union sum in the numerator. For this reason, the Dice metric and loss function is often utilized for medical image segmentation.

\paragraph{Tversky Coefficient and Loss}

The Tversky coefficient is yet another similarity metric related to both the Jaccard and Dice coefficient with a different method of handling class imbalance in the task of medical image segmentation. 

The Tversky Coefficient is defined as in eq \ref{eq: tversky_c}

\begin{equation}
\begin{split}
\label{eq: tversky_c}
T = \frac{|P \cap G|}{|P \cap G| + \alpha \times |P \setminus G| + \beta \times |P \setminus G|}
\end{split}
\end{equation}

The full form of the loss function is defined as in eq \ref{eq: tversky_loss}.

\begin{equation}
\begin{split}
\label{eq: tversky_loss}
Loss = 1 - \frac{|P \cap G|}{|P \cap G| + \alpha \times |P \setminus G| + \beta \times |P \setminus G|}
\end{split}
\end{equation}

$\alpha$ and $\beta$ control the magnitude of penalties of false positive versus false negative errors in the pixel classification for segmentation. The range of $\alpha$ and $\beta$ must be such that $ \alpha + \beta = 1$. The Tversky metric provides a spectrum of methods to normalize the size of a two-way set intersection. $\alpha$ and $\beta$ are hyper parameters that can be tuned to produce optimal loss results on the data-set of interest. The Tversky index can be thought of as a generalized Dice index. We can transform the Tversky coefficient into a Dice coefficient by setting $ \alpha = \beta = 0.5$. 


\subsection{Results and Analysis}

In Table \ref{table:Vnet}, we present the results from tuning a VNet architecture with the various metrics discussed in the previous section, namely Jaccard, Dice, and Tversky. We observe that Tversky loss function provided the best score. This could be explained by the fact that for the Tversky loss function, we have the most control of how we want to weight class imbalance. Tuning these parameters positively affected the accuracy of the model.

\begin{table}[]
\centering
\begin{tabular}{lcccr}
\hline
Model        &  Jaccard Score & Dice Score & Tversky Score       \\ \hline \hline
3D VNet (lymph)     &  0.869  &     0.517  & 0.984 (placeholder) \\
3D DenseUNet &  --            &    ----    &      -----          \\
SOA          &   ---          &     0.72   & ----                \\

%SOA is from miccai lymph node segmentation 2016 paper
%http://www.cs.jhu.edu/~lelu/publication/miccai2016_110.pdf
\end{tabular}
\caption{Scores for MSD Liver Data-set with different Evaluation Metrics. }
\label{table:Vnet}
\end{table}



















==> 3D_seg_lymph/future_work.tex <==
\chapter{3D Medical Image Segmentation}
%%%%%%%%% Lymph node one %%%%%%%%%%%%%%%%%%

In recent times, the rise of deep learning models for 2D medical image segmentation has been very prevalent and successful. The same trend starting to be observed for 3D medical data. After discussing the implementations of deep learning models for 2D medical image segmentation, this chapter transitions to exploring and validating the considerations to take into account when developing deep learning models for 3D medical image segmentation. There are many advantages to 3D medical image data-sets. 3D data-sets offer spacial coherence, which is quite beneficial for segmentation tasks. Although 3D data is limited, it provides important information that can help a deep learning model learn more accurate segmentation parameters. However, although 3D data provides a rich information that could not gain from 2D data, 3D data poses many challenges and transitioning to the 3D space is far from trivial. This chapter presents important considerations for preprocessing data-sets and implementing an efficient 3D medical image segmentation model. The effectiveness of these considerations are evaluated by testing them on a abdominal lymph node data-set. A 3D VNet model is then trained using this data-set.

\section{Background and Data-set}

Lesion and organ segmentation of 3D CT scans is a challenging task because of the high shape and size variations of anatomy between different patients. Much like in the 2D case, discussed in Chapter 4, 3D medical images suffer from low contrast from surrounding tissue, making segmentation difficult.

An interesting application for 3D image imaging is the segmentation of CT scans of the human abdomen to detect swollen lymph nodes.  Lymph nodes are small structures within the human body that work to destroy harmful substances. They contain immune cells that can help fight infection by attacking and destroying germs that are carried in through the lymph fluid. Therefore, the lymphatic system is essential to the healthy operation of the body. The presence of enlarged lymph nodes is a signal to the onset or progression of a malignant disease or infection. Therefore accurate segmentation models is critical to catch life threatening diseases at an early stage and support further treatment options.
The task of detecting and segmenting swollen lymph nodes in CT scans comes with a number of challenges. 
One of the biggest challenges in segmenting CT scans of lymph nodes in the abdomen is that the abdominal region exhibits exceptionally poor intensity and texture contrast among neighboring lymph nodes as well as the surrounding tissues, seen in Figure \ref{fig:3d_lymph}. Another difficulty is that low image contrast makes boundary detection between lymph nodes extremely ambiguous and challenging \cite{nogues2016automatic}. 3D lymph node segmentation is just one example out of the of many challenging 3D medical image segmentation problems. 


%In this this chapter, we focus on the task of liver segmentation in 3D CT Scans. In CT scans, the liver tissue is often difficult to identify because in the image, the intensity is similar to other organs around it, as can be seen in Figure \ref{fig:3d_lymph}. This makes liver segmentation a very challenging problem. Automated segmentation is initially the first step in health evaluation, early disease detection and clinical treatment such as radiotherapy or computer assisted surgery. The ability to accurately isolate and segment the liver can be of incredible assistance in the clinical process. In this chapter, we utilize the liver data-set from the Medical Segmentation Decathlon (MSD) Challenge. For this task, given a 3D CT scan, we utilize a VNet to segment out the swollen lymph nodes in CT scans.




%The following U-Net like 3D encoder-decoder architecture is presented to tackle this challenging yet clinically relevant issue by presenting an efficient light-weight deep learning architecture for 3D segmentation.

% \begin{figure*}
%   \includegraphics[width=\textwidth]{Images/3d_lymph.png}
%   \caption[Examples of Lymph Node Segmentation.]{(a) Examples of the top, side and front view of the original CT scan (b) Examples of the ground truth mask (red) overlaid on top of the CT scans. In the original image, the contrast is so low it is difficult to distinguish the lymph node segment even with the human eye.}
%   \label{fig:3d_lymph}
% \end{figure*}

\begin{figure}
\centering
\begin{tikzpicture}
\node (A) {\includegraphics[width=\linewidth]{Images/3d_lymph.png}};
\path (A.south west) -- (A.south east) node[pos=.15, below] {(1)} node[pos=.37, below] {(2)} node[pos=.65, below] {(3)} node[pos=.87, below] {(4)};
\node (B) {\includegraphics[width=\linewidth]{Images/3d_lymph.png}};
\path (A.north west) -- (A.south west) node[pos=.26, below] {(a)} node[pos=.76, below] {(b)};
\end{tikzpicture}
\caption[Examples of Lymph Node Segmentation.]{Examples of the top (a1,a3), side (a2,a4) and front view (b2, b4) CT scans. The ground truth masks are depicted in red (b1,b3). The low contrast in the CT scans make distinguishing the lymph node from the surrounding tissue a difficult task, even for the human eye.}
  \label{fig:3d_lymph}
\end{figure}


%REPHRASE https://arxiv.org/ftp/arxiv/papers/1812/1812.01049.pdf

\section{3D Data Preprocessing Techniques}

When developing a 3D segmentation architecture, there are several key points to consider. The first is the preprocessing techniques to be used on the data-set of interest. This includes image orientation (since we are not working in the 3D space), normalization methods, and how to fit large 3D images into memory. Another important consideration that makes quite a bit of difference in performance for 3D segmentation is the loss function that is utilized for training. The following sections describe these considerations in more detail so that the 2D medical image segmentation work presented in chapter 4 can be extended to the 3D domain in the future.

As mentioned above, segmentation in 3D offers a rich variety of information, as opposed to 2D segmentation. However, 3D segmentation does come with a number of considerations to take into account, as listed below. Each will be described in more detail in subsequent sections.:

\begin{enumerate}
\item \textbf{Consistent Orientation Across Images}: Orientation is important in the 3D space. Orienting all images in the same way while training reduces training time because it does not force the model to learn all orientations for segmentation. 
\item \textbf{Normalization}: This is a key step and there are differing techniques for different modalities.
\item \textbf{Generating Segmentation Patches}: This is an important strategy to use if there are memory constraints, which is often the case for 3D medical images. This strategy also aids in the issue of class imbalance in data-sets.
\item \textbf{Loss Functions and Evaluation Metrics}: Loss functions are important considerations for 3D segmentation and can also aid in the issue of class imbalance in data-sets.
  %\item One of the biggest challenges faced is the amount of memory available to run models. In our case, we had one 11GB Nvidia 1080x GPU and each raw image was 512 by 512 by 775. This was way too large to fit an entire image plus a simple 3D UNet.
  %\item Class imbalance is another issue, since within each sample, the background dominated the foreground. Therefore during training, the model was prone to overfit to the background class.
  %\item Training time took much longer since there were more voxels (3D version of pixels) contributed to the calculation of the gradient and back propagation.
\end{enumerate}

The lymph node data-set was fed through the following pipeline in Figure \ref{fig:preprocess} to alleviate the issues listed above and properly preprocess the 3D data. The next sections describe the preprocessing steps in more detail.

\begin{figure}
  \includegraphics[width=\linewidth]{Images/preprocess.png}
  \caption{Proprocessing Pipeline for 3D Data-set.}
  \label{fig:preprocess}
\end{figure}

\subsection{Consistent Orientation Across Images}

In 3D images, the idea of orientation becomes an issue of interest. Consistent orientation among all images is important to speed up training time. If there are multiple orientations, the network is forced to learn all orientation, and in order to generalize, more data is required, which is not easy to come by for 3D medical images. Nibable, which is an open source python library to read in medical images, is utilized to determine 3D image orientation and reorient images, if required. It was found that the orientation selection itself did not make a difference on training as long as the orientation was consistent throughout the data-set. 

\subsection{Normalization}

Normalization is a key step in the preprocessing pipeline for any deep learning task. Normalization is also very important for medical images and there are varying methods of doing this. The aim of normalization is to remove heavy variation in data that does not contribute to the prediction process and instead accentuate the features and differences that are of most importance. There are a few interesting methods that could be used specifically for medical image segmentation such as the following \cite{dltk_overview}:
\begin{enumerate}
  \item Voxel Intensity Normalization:   
  Voxel intensity Normalization is very dependent on the imaging modality. For images such as weighted brain MR images, a zero-mean unit variance normalization is standard procedure. This is done because the contrast in the image is usually set by an expert taking the MRIs and thus there is high variation in intensity based on user across image sets. This variation can be considered noise. Thus to get rid of this noise and standardize intensity across multiple intensity settings, we use a zero mean normalization. In contrast, CT imaging measures a physical quantity such as radio-density in CT imaging, where the intensities are comparable across different scanners. Therefore, for this modality, the standard normalization methodology is clipping or rescaling to a range such as [0,1] or [-1,1].
  
  \item Spacial Normalization:
   Normalizing for image orientation avoids the need for the model to learn all possible orientations of input images. This reduces both the need for a large amount of training data and training time. Since, as mentioned before, properly labeled medical data is often small in quantity, this is a very effective technique of normalization.  
\end{enumerate}

%FIX THIS
Since the the modlaity of the abdominal lymph node data was 3D CT scans, both methods of normalization were used. Reorientation was also done on all images. Voxel intensity normalization was performed by rescaling all voxels in the images to a range of [-1,1] and the voxels in the labels to [0,1].

\subsection{Generating Segmentation Patches}

Patch based segmentation is used to tackle the issue of limited memory. A single 3D image in the lymph node data-set was 512 by 512 by 775. With the memory constraints, using these raw images would only allow for a batch size of 1, which would result in an incredibly long training time, and very little flexibility to extend the deep learning architecture. Therefore patch based segmentation was utilized. 

The basic idea of patch generation is to take in an input image, determine the regions of most interest in the image, and return a smaller portion of the image, focusing on these regions of importance. Doing this is important for many reasons. The first reason is, having smaller image sizes allow for larger batch sizes and faster training. The second reason is that the data is naturally augmented with this process. The third reason is that class imbalance issues can be avoided. Class imbalance occurs when a sample image has more voxels belonging to one class over another. Figure \ref{fig:3d_lymph}b shows this very clearly. In the example, the majority of the voxels belong to the background (black) class and a small subset belong to the foreground (red) class. Feeding such images directly to the model will cause the the model to skew its learning to favor the background voxles. Therefore, intelligent selection of patches is key to training. For this work, we generated patches of 128 by 128 by 128. We utilized the Deep Learning Toolkit to generate our class balanced segmentation patches. %maybe expand more with diffferent patch selection techniques or explain the DLTK one

Unlike during training time, in which the patches are generated randomly around areas of interest, during test time, the images is systematically broken into 128 by 128 by 128 chunks. Prediction is done on each chunk and the chunks are joined together for the final prediction. The patching technique alone, creates some discrepancies at the boarders of patches so smoothing is performed to get a more seamless prediction.

\subsection{Loss Functions and Evaluation Metrics}

%For the VNet architecture, we decide to experiment with different loss functions to see how it affects the performance of the model.
The choice of loss functions can significantly affect the performance of 3D segmentation architectures. Loss functions are discussed in more detail to gain some intuition for why one would produce better results over another.

In medical images, it is very common that the region of interest,for example, a lesion or an organ, covers a very small portion of the scan. Therefore, during the learning process, the network often gets stuck in local minima due to this class imbalance of background and foreground pictures. This causes poor results during training and testing since the prediction of both classes is weighed equally. This causes the model to be biased toward the background voxels and the foreground is either completely missed or partially detected. The following losses attempt to address these issues.

% \begin{figure}
%   \includegraphics[width=\linewidth]{Images/preprocess.png}
%   \caption{Proprocessing Pipeline for 3D Data-set}
%   \label{fig:preprocess}
% \end{figure}

\paragraph{Jaccard Coefficient and Loss}

The Jaccard coefficient is measure of similarity between a ground truth mask and a prediction mask. Lets assume that all voxels in the ground truth mask are in set $G$. All voxels in the prediction mask are in set $P$. The Jaccard coefficient calculates the ratio of 3 mutually exclusive partitions: $|P \cap G|$, $|P \setminus G|$, $|P \setminus G|$. The equation for the Jaccard coefficinet is seen in eq \ref{eq: jaccard_c}.
\begin{equation}
\begin{split}
\label{eq: jaccard_c}
J = \frac{|P \cap G|}{|P \cap G| + |P \setminus G| + |P \setminus G|}
\end{split}
\end{equation}

The full loss function is defined as in eq \ref{eq: Jaccard_loss}.

\begin{equation}
\begin{split}
\label{eq: Jaccard_loss}
Loss = 1 - \frac{|P \cap G|}{|P \cap G| + |P \setminus G| + |P \setminus G|}
\end{split}
\end{equation}

The Jaccard coefficient calculates the overlap ratio between a ground truth mask and a predicted mask by giving equal weightage to  $|P \cap G|$, $|P \setminus G|$, $|P \setminus G|$. If the data of interest does not suffer too much from class imbalance, the Jaccard coefficient and loss is a good metric to measure the success of a model. If there is class imbalance, this method may not produce as promising results and a model could become biased towards the dominating class. 

\paragraph{Dice Coefficient and Loss}

The Dice coeffient is another metric that compares the similarity between a ground truth mask and a prediction mask. It is similar to the Jaccard coefficient with one subtle but significant difference in the way class imbalance is handled. Dice Loss is used in Chapter 4, as it is a widely uses loss function for both 2D and 3D medical image segmentation. The Dice coefficient, also known as the Sorensen-Dice coefficient, is defined as in eq \ref{eq: Dice_c}

\begin{equation}
\begin{split}
\label{eq: Dice_c}
D = \frac{2 \times |P \cap G|}{2 \times |P \cap G| + |P \setminus G| + |P \setminus G|}
\end{split}
\end{equation}

The full Dice Loss is as in eq \ref{eq: Dice_loss}. $|P \setminus G|$ notation refers to the set of elements in $P$ but not in $G$.

\begin{equation}
\begin{split}
\label{eq: Dice_loss}
Loss = 1 - \frac{2 \times |P \cap G|}{2 \times |P \cap G| + |P \setminus G| + |P \setminus G|}
\end{split}
\end{equation}

The Dice coefficient is a measure of similarity between two sets. The Dice Coefficient addresses the issue of class imbalance by calculating the overlap between a prediction and a ground truth mask for a region of interest. The Dice coefficient is unique because unlike the Jaccard metric, the Dice metric gives more weight to voxels that belong to both sets (aka the overlapping region of both sets) when calculating the overlap ratios, hence the factor of 2 that is multiplied to the union sum in the numerator. For this reason, the Dice metric and loss function is often utilized for medical image segmentation since correct overlapping regions are hard to find due to irregular lesion shapes.

\paragraph{Tversky Coefficient and Loss}

The Tversky coefficient is yet another similarity metric related to both the Jaccard and Dice coefficient with a different method of handling class imbalance in the task of medical image segmentation. 

The Tversky Coefficient is defined as in eq \ref{eq: tversky_c}

\begin{equation}
\begin{split}
\label{eq: tversky_c}
T = \frac{|P \cap G|}{|P \cap G| + \alpha \times |P \setminus G| + \beta \times |P \setminus G|}
\end{split}
\end{equation}

The full form of the loss function is defined as in eq \ref{eq: tversky_loss}.

\begin{equation}
\begin{split}
\label{eq: tversky_loss}
Loss = 1 - \frac{|P \cap G|}{|P \cap G| + \alpha \times |P \setminus G| + \beta \times |P \setminus G|}
\end{split}
\end{equation}

$\alpha$ and $\beta$ control the magnitude of penalties of false positive versus false negative errors in the pixel classification for segmentation. The range of $\alpha$ and $\beta$ must be such that $ \alpha + \beta = 1$. The Tversky metric provides a spectrum of methods to normalize the size of a two-way set intersection. $\alpha$ and $\beta$ are hyper parameters that can be tuned to produce optimal loss results on the data-set of interest. The Tversky index can be thought of as a generalized Dice index. We can transform the Tversky coefficient into a Dice coefficient by setting $ \alpha = \beta = 0.5$. 

\section{3D VNet Implementation and Data Processing Pipeline}

%%%% FIX REFF %%%%
The base implementation of this VNet architecture was inspired by the work by \cite{jackyko1991_vnet_tensorflow}. The main portions of this architecture involved a data-loader, the VNet model, and an evaluation pipeline, to see how well the model can predict on new images. However, many changes had to be made to the pipeline. 
In medical imaging, data input-output is often one of the most challenging steps. This is especially challenging for the case of 3D images, since special care must be taken to load and preprocess the data. The initial data-loader and training pipeline involved using the SimpleITK package to read in, normalize, and randomly select patches to train the model on. The disadvantage to using SimpleITK is that this library does not utilize GPU accelerated operations, making the data-loader slow and inefficient. SimpleITK was also utilized for the evaluation pipeline. Since SimpleITK is not GPU compatible, memory constraints were an initial problem. Therefore, data-loader and evaluation pipelines were then changed to utilize the Nibabel and Deep Learning Toolkit (DLTK) packages. The Nibabel package was used to read in a image, normalize the image, and make all image orientations. The DLTK package was used to select patches to train the model on. DLTK utilizes an algorithm that determines the regions of interest in each image and creates patches around this region to promote class-balanced samples. This improved end-to-end pipeline was utilized to train the VNet model to predict swollen lymph nodes give 3D abdominal CT scans. 


\subsection{Results and Analysis} %%%%% FIX THIS WITH SOME PICTURES

% \begin{figure*}
%   \includegraphics[width=\textwidth]{Images/lymph_final.png}
%   \caption[3D Segmentation Results with VNet architecture and Dice Loss.]{(a)Examples of segmentation overlaid with ground truth masks. (b) Examples of segmentation overlaid with predicted masks. In each set of 4 images, the top left is a top view, top right is a side view, bottom left is the segmentation mask, bottom right is a front view. (1) shows results from a few hours of training. (2) show results from a few days of training.}
%   \label{fig:lymph_final}
% \end{figure*}

\begin{figure}
\centering
\begin{tikzpicture}
\node (A) {\includegraphics[width=\linewidth]{Images/lymph_final.png}};
\path (A.south west) -- (A.south east) node[pos=.29, below] {(1)} node[pos=.73, below] {(2)};
\node (B) {\includegraphics[width=\linewidth]{Images/lymph_final.png}};
\path (B.north west) -- (B.south west) node[pos=.25, below] {(a)} node[pos=.73, below] {(b)};
\end{tikzpicture}
\caption[3D Segmentation Results with VNet architecture and Dice Loss.]{(a)Examples of segmentation overlaid with ground truth masks. (b) Examples of segmentation overlaid with predicted masks. In each set of 4 images, the top left is a top view, top right is a side view, bottom left is the segmentation mask, bottom right is a front view. (1) shows results from a few hours of training. (2) show results from a few days of training.}
  \label{fig:lymph_final}
\end{figure}

%%%%%%%%%%%%%%% FIX CAPTION %%%%%%%%%%%%%%%%
% \begin{table}[]
% \centering
% \begin{tabular}{lcccr}
% \hline
% Model         & Dice Score      \\ \hline \hline
% 3D VNet (lymph) &  0.0038


% %SOA is from miccai lymph node segmentation 2016 paper
% %http://www.cs.jhu.edu/~lelu/publication/miccai2016_110.pdf
% \end{tabular}
% \caption{Dice Score for Abdominal Lymph Node Data-set.}
% \label{table:Vnet}
% \end{table}

Figure \ref{fig:lymph_final} shows very preliminary results of this model on the lymph node data-set. For the preliminary result the 3D VNet model was trained using a Dice loss function. (a) depicts the CT scans overlaid with the ground truth masks. The lower left depicts the 3D isolated lymph nodes. (b) depicts the CT scans overlaid with the predicted masks from this VNet architecture. Again, the loser left images show the isolated 3D mask prediction. For (a), it is evident how difficult this problem is, due to small size of the lymph nodes, compared to the rest of the body. These preliminary results were obtained by training (1) for a few hours and (2) for a few days. An interesting observation is that even within a few hours, the VNet started to distinguish boundaries in the image, which explains why the bottom left image in (b1) look like the outline of the patient in 3D. After training the model for a few days, it was observed that even more details are learned by the VNet, such as the ribs (b2). This trend suggests that if the model was trained long enough, it would start to pick up the nuances of the lymph nodes. However, this also suggests that there are many improvements that could be made to this model to allow for better performance, such as adding dense connectivity to the VNet, similar to the 2D version in Chapter 4, different loss functions, or different styles of encoder-decoder architectures. Due to time constraints, exhaustive evaluation metrics and trials on the effects of different loss functions for this data-set were unable to be performed. However, this work has set the foundation for many future endeavors and extensions of this work, as discussed in the next section.

\section{Future Work}

%different loss functions can be used
%extending the architecture (different types of autoencoders)
%longer training time
%more computational resources.

The work discussed in the previous sections of this chapter set the foundation for developing a robust 3D model for medical image segmentation. There are many suggested improvements to this model, including exploring additions to the basic VNet architecture, how different loss functions affect training, or experimenting with the effectiveness of using more computational resources, if available.

\subsection{Additional Loss Functions}

For the VNet model describes above, a Dice loss function was utilized. This was chosen because it is the most cited metric for the case of medical image segmentation. However, one can experiment with other loss functions, such as the ones discussed in the loss function section, to see which one is most effective at handling class imbalance in data-sets. For the case of lymph node segmentation, there was heavy class-imbalance, as observed in Figure \ref{fig:lymph_final} a. Therefore, another useful loss function to explore could be the Tversky loss function. Weighted Cross Entropy is yet another effective loss function utilized in more general segmentation tasks.

%layers loss functions, collect losses after different layers


\subsection{Additions to the VNet Architecture}
%dense blocks, dilations 
%different encoder-decoder scheme

The first suggested modification, in conjunction to the previous chapters of this work, is to experiment with adding dense blocks to this VNet architecture. As seen in the 2D case, it is reasonable to hypothesize that adding dense connectivity will increase the learning capabilities of the model because each layer will directly take as input all previously learned feature maps. For challenging segmentation tasks, such as swollen lymph node segmentation, it is observed that the learning process is rather slow. Dense connectivity could also help speed up the learning process due to easier flow of gradients during back propagation. Another suggested modification to the VNet architecture is to add dilated convolutions to gain spacial awareness on the encoder side of the VNet. Dilated convolutions can be useful in the 3D case because they are computationally efficient with the advantage of an expanded receptive field, which is critical in the 3D case. 

\subsection{Additional Computational Resources}

All of the work discussed in this thesis utilized one Nvidia 1080 Ti GPU. This was a powerful resource to effectively train the 2D models on 256 by 256 images, developed in Chapters 3 and 4. For the case of the 3D data-set, the image sizes varied from 512x by 512 by 48 to 512 by 512 by 775. These images were much too large to fit more than one into memory at a time. Therefore, a patch based method was adopted to train the model for segmentation. Although in the preliminary results suggest the potential effectiveness for the patch based approach for training, with more computational resources to feed an entire image in at a time for training, it's reasonable to hypothesize that even a basic VNet model would be much more effective and robust. Regardless of this computational resource limitation with regard to the 3D space, this work demonstrates a series of highly effective 2D models and sets the foundation for the extending models into the 3D space for medical image analysis.


















==> Conclusion/conclusion.tex <==
\chapter{Conclusion}

Image segmentation is a topic of great interest in computer vision and has been utilized for a number of tasks, such as object localization, boundary detection, medical imaging, and recognition. Prior successful segmentation methods relied on a user initialization, to some extent . This work proposed effective architectures to \textit{fully automate the process of localizing and delineating boundaries} of objects in images. This research work developed and implemented deep learning frameworks for two segmentation tasks, namely salient object detection and 2D binary medical image segmentation. The work also explored and evaluated the considerations that should be taken into account when moving from 2D medical image segmentation to 3D. This set the foundation to extend the 2D models discussed in this work to the 3D space in the future.

First, the problem of salient object detection was tackled, to gain a basic understanding of segmentation. A number of iterations of encoder-decoder architectures were described before arriving at a novel dense dilated encoder-decoder network with dilated spatial pyramid pooling. This work was used as the backbone CNN architecture for an ICML 2019 submission, for initial object localization and boundary detection. The full pipeline outperformed one of the three popular data-sets used for salient object detection, and was very competitive with the other two data-sets. The segmentation results of the dilated dense encoder-decoder were also impressive, indicating that this architecture could be used as a robust stand alone segmentation architecture as well.

Next, an important and relevant use case of segmentation was addressed, namely 2D medical image segmentation. A novel dilated dense UNet architecture was developed and implemented to combat the many challenges faced with 2D lesion segmentation, such as low image contrast, lack of large labeled data-sets, and the lack of robust pretrained models. A custom data-set from a collaboration with Stanford University was utilized to evaluate this model’s performance. When comparing the results of training and testing the dilated dense UNet model to the baseline, the dilated dense UNet demonstrated significant increase in performance, confirming the effectiveness of the architecture. This work was used as the backbone CNN for a CVPR 2019 submission, for accurate initial lesion localization and boundary delineation. The segmentation results of the stand alone dilated dense UNet also showed promising results for 2D lesion segmentation, suggesting that it is capable of performing well on its own.

The purpose of this work was to develop deep learning models to address the challenges faced when performing salient object segmentation and 2D medical image segmentation. To combat the challenges faced in each task, two main architectures were proposed for automated object localization and boundary delineation. This work also discussed the considerations to be taken when extending 2D medical segmentation models into the 3D space, so that this research could  be extended in the future to develop robust 3D architectures for medical image segmentation. Extending the 2D architecture would be effective since most raw medical images are in the 3D domain.

In the recent past, a number of tasks dependent on image segmentation have come to light, such as medical imaging, autonomous driving, or scene understanding. This research work hoped to gain a deeper understanding of image segmentation and contribute to this topic, which has become critical to understanding and assisting the world around us.




==> Image_Seg/image_seg.tex <==
\chapter{Image Segmentation}

\section{Overview}
\section{Medical Images}
\section{Dataset}
Since the Stanford Data-set is comprised of different organs across various image modalities such as CT and MRI, we trained the Deep Level Sets on each of them separately and evaluated its performance on their corresponding test sets. Furthermore, we also trained the FCN backbone of Deep Level Sets, namely Dilated Dense U-Net, in addition to a comparable U-Net models in order to measure the effectiveness of the active contour layer. We used the Dice coefficient for measuring the similarities between the predictions and labels. Results of these studies are presented in Table ####

==> Intro/intro.tex <==
\chapter{Introduction}

%What is image segmentation
%binary image segmentation for medical image, saliency object detection for natural images, semantic segmentaiton for natural images
%why is a significant problem 
%medical image segmentation 
%natural image segmentation 

% \begin{figure}
%   \includegraphics[width=\linewidth]{Images/img_seg.png}
%   \caption[Types of image segmentation discussed in this work.]{(a) Example of natural image (left) and its corresponding salient object map (right). (b) Example of 2D brain MRI (left) and the corresponding lesion segmentation map (right). (c)Example of 3D liver CT from top, side and front perspectives (left) and corresponding liver segmentation maps for top, side and front perspectives (right). Liver is highlighted in red on the original CT (left).}
%   \label{fig:img_seg}
% \end{figure}

\begin{figure}
\centering
\begin{tikzpicture}
\node (A) {\includegraphics[width=\linewidth]{Images/img_seg.png}};
\path (A.south west) -- (A.south east) node[pos=.18, below] {(a)} node[pos=.52, below] {(b)} node[pos=.83, below] {(c)};
\end{tikzpicture}
\caption[Types of image segmentation discussed in this work.]{(a) Example of natural image (left) and its corresponding salient object map (right). (b) Example of 2D brain MRI (left) and the corresponding lesion segmentation map (right). (c)Example of 3D liver CT from top, side and front perspectives (left) and corresponding liver segmentation maps for top, side and front perspectives (right). Liver is highlighted in red on the original CT (left).} 
  \label{fig:img_seg}
\end{figure}

Image segmentation is a prominent concept of computer vision. It is the process of partitioning the pixels in an image into different classes, or segments. The main goal of segmentation is often to simplify the representation of an image such that it is easier to interpret, analyze and understand. Image segmentation has been classically used in a variety of computer vision task, such as object localization, boundary detection, medical imaging, and recognition tasks. In essence, these tasks are done by assigning each pixel in an image to a certain label based on similar attributes, such as texture, color, intensity, or distance metrics. The result of image segmentation is a set of segments that collectively cover the entirety of an image. There are several types of segmentation tasks. This work will mainly explore and discuss novel deep learning methods for salient object segmentation on natural images and 2D and 3D binary medical image segmentation.

%salient object detection overview what it is and significance
There are two types of segmentation discussed in this work. The first is salient object segmentation. Salient object segmentation on natural images, is the detection of the most prominent, noticeable, or important object within the image. Therefore, salient object segmentation is an intuitive first step to explore the field of image segmentation. In computer vision, the goal of a saliency map is to classify each pixel in the image as being part of the salient object or part of the background. Figure \ref{fig:img_seg}a illustrates an example of an image and its associated salient map. The reason for dividing images into either the salient object or the background is to simplify the representation of the image and make it easier to analyze. Salient object segmentation is especially important because it assists in making applications smarter by learning the most important aspects of an image. An example use case is smart image cropping and resizing. Salient object segmentation is used to understand the most relevant portions of the image and then the image can be automatically cropped without losing this information. Another use case is in UI/UX design \cite{salient}. In UI/UX design, salient object segmentation is used to understand what parts of a user interface are most useful. This information can help support the development of even better user interfaces for a more smooth user experience. Salient object segmentation is a mechanism to automate the process of determining the most important parts of images and this, in turn, supports a number of other product pipelines. 

%medical image - overview what it is and significance
After exploring salient object detection on natural images, we shift the second important and relevant use case for image segmentation, namely medical image segmentation. Medical image segmentation is the process of automatic detection of lesions or cancerous boundaries within 2D or 3D medical images. In this work, we use binary medical image segmentation to detect lesions in 2D MRIs and CT scans of the brain and lung. We also segment swollen lymph nodes in 3D CT scans. The goal, whether for 2D or 3D images, is to create a model that can accurately segment a lesion, organ, or cancerous region in a CT or MRI scan. Figure \ref{fig:img_seg}b and c shows examples of lesion segmentation in 2D and 3D images. Medical image segmentation comes with many challenges that we did not face in salient object detection on natural images. Some examples include, lack of large data-sets, specialized preprocessing techniques on different modalities of medical imaging, memory constraints with 3D medical images, and the inability to use priors on the shapes of lesions and organs because they are so unique to each patient. Although a difficult task, medical image segmentation is a significant part of computer vision for many reasons. For one, having a robust and reliable method of detecting the presence of severity of a disease will positively impact clinical care. Medical image segmentation is often the first step in a diagnosis analysis plan. Therefore, accurate segmentation is a key step in treatment planning \cite{aggarwal2011role}.

%Brief related work
Traditionally, energy based models have been successfully applied for the task of image segmentation \cite{kass1988snakes,zhu1996region,osher2001level}. These models rely on the content of the image and minimize an energy functional that corresponds to the contour that guides the segmentation process. Furthermore, with the ever-increasing computational power, availability of data and universal function approximation capabilities of neural networks \cite{hornik1989multilayer}, deep learning methods have become ubiquitous in many applications \cite{hatamizadeh2018optimizing,nakada2018deep}, and deep convolutional neural networks have achieved state-of-the-art results on bench-marked data-sets for various image recognition tasks in recent years \cite{krizhevsky2012imagenet,simonyan2014very,he2016deep}. Image segmentation has benefited from various powerful fully convolutional architectures that can produce output predictions of the same size as the input image \cite{badrinarayanan2015segnet}, and the proposed encoder-decoder architectures such as UNet \cite{ronneberger2015u} allow for re-using the learned representations of the encoder and better localizing the objects in the decoder.

%brief problems with related work
Although the current deep-learning assisted models for image segmentation have achieved acceptable results in many domains, these models are yet incapable of producing segmentation outputs with precise object boundaries. This work aims to improve this current paradigm by proposing novel architectures for better delineation of object boundaries. In addition to the capability of the proposed architectures to be used as a standalone model, they can also be leveraged in an integrated framework with other energy-based components with the goal of decreasing the user dependency of such models on external inputs as well as improving their robustness. 

%our solutions/contributions
We first tackle the problem of salient object detection and segmentation in natural images and propose an effective architecture for localizing and delineating boundaries of appearing object. We then investigate the problem of cancerous lesion segmentation and address the issues previously discussed in various 2D medical imaging data-sets that contain lesions of different size and shape. Finally, we explore the preprocessing considerations that should be taken into account when transitioning from 2D segmentation model to the 3D space. We evaluate these considerations by preprocessing a abdominal lymph node data-set. We then train and fine-tune that 3D VNet model using the preprocessed data-set. The 2D architectures presented in this work (Chapters 3 and 4) were used as a backbone in an integrated framework in submissions to 2019 International Conference on Mass Data Analysis of Images and Signals (MDA) and  International Conference on Medical Image Computing and Computer Assisted Intervention (MICCAI).


The remainder of this thesis is organized in the following way. 
\begin{itemize}
\item In Chapter 2, techniques that were popular for image segmentation prior to deep learning methods are discussed. The transition to the utilization of deep learning methods are then highlighted. Three deep learning architectures which inspired the work for this thesis are also discussed in detail, namely UNet, DenseNet and VNet.
  \item In Chapter 3, a novel architecture for the task for salient object segmentation is introduced. The highlights of this architecture include, an custom encoder-decoder architecture with dense blocks and a dilated spacial pyramid pooling unit for better spacial understanding in images.
  \item In Chapter 4, a more specific use case for image segmentation is explored, namely medical image segmentation. A novel deep learning architecture for 2D medical image segmentation on a new medical image data-set from Stanford University is discussed. The highlights of this architecture are an encoder-decoder network with dense blocks which compete with the state-of-the-art with very limited data.
  \item In Chapter 5, important considerations required to transition from a 2D segmentation model to a 3D segmentation model are discussed. The importance of preprocessing techniques in the 3D case is highlighted. A 3D medical data-set is preprocessed using these techniques and a 3D VNet is trained and fine-tuned with the processed data.

\end{itemize}

The purpose of this work was to explore different deep learning techniques for both natural and medical image segmentation. This included designing and implementing novel deep learning architectures to improve the automation of delineation for boundaries for segmentation as well as exploring and utilizing current state-of-the-art architectures for the tasks of salient object segmentation and medical image segmentation. In recent years, there have been many efforts in computer vision, such as medical imaging, autonomous driving, traffic control systems and various recognition tasks, which rely on some sort of segmentation task. This work explored deep learning methods for image segmentation in the hopes of supporting these future efforts.


==> Makefile <==

#
# uclathes Makefile
# Copyright (C) 1995 by John Heidemann, <johnh@isi.edu>
#

FILES=README \
	demo.tex demo.dvi demo.pdf \
	demo_techreport.tex demo_techreport.pdf \
	thesis_spec.tex thesis_spec.pdf \
	uclathes.cls uclath12.clo uclathti.clo uclathma.clo \
	uclathes.bst Makefile

all:  latex ps pdf

tar: $(FILES)
	tar cvf uclathes.tar $(FILES)

tar.gz:
	@echo "Make all before doing make tar.gz"
	tar czvf uclathes.tar.gz $(FILES)

DVIPS=dvips
PS2PDF=ps2pdf14

latex latex.demo::
	latex demo

ps demo.ps::
	$(DVIPS) demo

pdf demo.pdf::
	$(PS2PDF) demo.ps demo.pdf

latex latex.demo_techreport::
	latex demo_techreport

ps demo_techreport.ps::
	$(DVIPS) demo_techreport

pdf demo_techreport.pdf::
	$(PS2PDF) demo_techreport.ps demo_techreport.pdf

latex latex.thesis_spec::
	latex thesis_spec

ps thesis_spec.ps::
	$(DVIPS) thesis_spec

pdf thesis_spec.pdf::
	$(PS2PDF) thesis_spec.ps thesis_spec.pdf

clean:
	rm *.aux *.toc *.lot *.lof *.dvi *.log *.ps


==> Related_Work/related_work.tex <==
\chapter{Related Work}
%techniques used for segmentation in the past
%for medical images
%for natural image

%Ideally, in order to achieve state-of-the-art results with the deep learning approaches we will discuss, we require large data-sets to allow models to learn features and perform segmentation well. The lack of data availability is a huge drawback in medical image segmentation. In this work, we discuss how to alleviate the problem of limited data by presenting a novel encoder-decoder architecture for 2D and 3D medical image segmentation. In traditional feed-forward convolutional neural networks with large data-sets, the model has the luxury of learning little bits of information over a vast number of examples and aggregates all that information into a generalized model. In the case of medical image segmentation, where there is a lack of data, our model needs to maximize the information learned from each example we have. Our encoder-decoder architecture is effective even with small data-sets because unlike feed-forward convolutional neural networks, in which each layer only gets the receptive fields (feature maps) from the previous layer, our encoder-decoder structure's receptive fields on the encoder side are concatenated with the receptive fields on the decoder side. In addition, every layer is takes as input all the feature maps learned from all previous layers via dense blocks for maximal imformation gain per convolution. This results in a model that has an overall greater understanding from a data-set in which a model has limited examples to learn and generalize. This maximal learning strategy via increased receptive fields has shown better performance over a classical feed-forward network that has limited receptive fields from only previous layers. More information at each step of the convolution allows for better feature learning. To increase spacial understanding, we also include dilation in our convolutions to further increase receptive fields at reduced resolutions and understand where objects are relative to other objects during segmentation. Medical image segmentation is a significant part of computer vision for many reasons. For one, having a robust and reliable method of detecting the presence of severity of a disease will positively impact clinical care. Medical image segmentation is often the first step in a diagnosis analysis plan. Therefore, accurate segmentation is a key step in treatment planning \cite{aggarwal2011role}.

This related work discusses segmentation techniques that have been explored prior to the rise of deep learning for segmentation. Three noteworthy deep learning architectures that inspired the work in this this thesis are then mentioned, nemely UNet, DenseNet, and VNet.

\section{Salient Object Segmentation on Natural Images}

Salient object segmentation is the task of detecting the most prominent object in an image and classifying each pixel in an image as either part of that object or part of the background (a binary classification task). Before deep learning methods, there were five main categories of methods for the problem of image segmentation, namely region-based methods, classification methods, clustering methods, hybrid methods, discussed in \cite{norouzi2014medical}, and active contour models. For each method, the algorithm is described, followed by the advantages and disadvantages of the algorithm.

There are two main region-based methods, thresholding and region growing. Thresholding is a simple segmentation approach, first discussed in the work by \cite{bogue2005machine}, that divides the image into different segments based on different thresholds of pixel intensity. In other words, this method assumes that, given an image, all pixels belonging to the same object have similar intensities, and the overall intensities of different objects differ. Therefore, every pixel can be classified in this manner. Global thresholding assumes that the pixel distribution of the image is bi-modal. In other words, there is a clear difference in intensity between background and foreground pixels. However, this naive global method performs very poorly if the image has a lot of noise and the pixel intensity per region has low variability, since these thresholds were initially determined visually by a user. More sophisticated global thresholding techniques include  Otsu's Thresholding by \cite{qu2010research}. This method assumes a two pixel class image in which the thethreshold value aims to minimize the intra-class variance. Local thresholding helps this issue by dividing images into subimages and determines a threshold value for that region. The resultant is then combined together to get the final segmentation. Local thresholding is achieved using different statistical techniques, including calculating the mean, standard deviation, or maximum/minimum of a sub region. An even more sophisticated method of thresholding is region growing. This method requires an initial seeds that grows due to similar properties for surrounding pixels, representing an object, as done in \cite{leung1998contour}. The obvious drawback to this approach is that it is heavily dependent on the selection of the seeds by a human user. Human interaction often results in a high chance of error and differing results based on different user nationalizations.

k-nearest neighbors and maximum likelihood are simple and prominent classification methods used prior to deep learning. K-nearest neighbors is a strategy in which for each image, pixels are assigned to different object classes based on classification learned at training time. The idea was first applied to medical images by \cite{korn1998fast}. The advantage to this model was that it was easy to train. The downfall of this technique is that it requires a large training set to learn the optimal nearest neighbor. In the medical domain, copious amounts of data is rare, therefore this method cannot prove to be heavily robust.

Clustering methods attempt to mitigate the issues faced in classification since clustering methods do not require a training set. This is favorable in the medical domain due to the lack of larger varied data-set. These algorithms use statistical analysis to understand the distribution and representation of the data, and and, therefore, are considered unsupervised learning approaches. Some examples of clustering include, k-means, fuzzy C-mean, and expectation maximization, as shown in \cite{med_lit_review}. The main disadvantage of clustering methods is that it is sensitive to noise since it does not take into account the spacial information of the data. It only cluster locally.

Hybrid methods are techniques that use both boundary (thresholding) and regional information (classification/clustering) to perform segmentation. Since this method combines the strengths of region-based, classification and clustering methods, it has proved to give competitive results out of the non deep learning techniques. One of the most popular methods is the graph-cut method. This method requires a user to select initial seed pixels belonging to the object and seed pixels belonging to the background. Then, it uses the minimum cut algorithm on the graph generated from the image pixels, as discussed in \cite{boykov2001interactive}. The drawback is the need for a user to select the initial seed. This is error prone for low contrast images and would be more advantageous if it could be automated.

%active contour models
Active contour models (ACMs), first developed by \cite{kass1988snakes} have been very popular for segmentation, as in \cite{vese2002multiphase} and object boundary detection, as in \cite{mishra2011decoupled}. Active contour models utilize formulations in which an initial contour evolves into the object's boundary, via the minimization of an energy functional. Level Set models are a type of active contour model. They are able to generate a continuous boundary of an object, and can handle variations in shape, image noise, heterogeneity, and discontinuous object boundaries, as shown in \cite{5754584}. This method is extremely effective if the initialization of the contours and weighted parameters is done properly. In the initial stages of level set methods, this contour initialization was done by hand, and hence tedious and prone to error. Researchers have proposed automatic initialization methods, such as using shape priors or clustering methods. Although these remove a manual initialization step, techniques like shape priors require a large representative amount of training data. This is difficult in the medical domain, not just because data is limited but also because every lesion is so unique to a given patient. Therefore it is challenging to predict the shape of a lesion to use as a prior.

For the task of salient object detection, we worked with natural images, and this task comes with certain advantages when compared to working with medical images. Natural images have much larger data-sets and the use of priors is possible, since the shape of basic objects are known such as animals, furniture, or cars. The idea of utilizing a prior was used by \cite{han2015background}. In this work, the authors propose a framework for salient object detection by first modeling the background and then separating salient objects from the background. \cite{hou2016deeply} proposed a CNN architecture that introduces short connections to the skip-layer structures within a Holistically-Nested Edge Detector architecture. 

%The recently proposed Deeplabv3+ \citep{chen2018encoder} has mitigated this problem to some extent by leveraging the power of dilated convolutions, but such improvements were made possible by extensive pre-training and vast computational resources---50 GPUs were reportedly used to train this model.

\section{2D and 3D Medical Image Segmentation}

Modern technology has allowed the production of high quality medical images to aid doctors in illness diagnosis. The first step after producing these images is to segment them into organs or lesions within the organs. Before the rise of computer vision in the medical domain, this segmentation was often done manually, where medical technicians would hand draw the boundaries of different organs and lesions. This process is not only tedious for technicians but also error prone, since getting accurate boundaries by hand can be rather tricky in some cases. In the past few decades, there have been many effective algorithms that have surfaced to aid in this process of segmentation. These models incorporate mathematics and physics to enhance the accuracy of segmentation, as discussed in \cite{med_lit_review}. Region-based methods, classification methods, clustering methods, hybrid methods and active contour models, mentioned in the previous section, were also utilized for medical image segmentation prior to the rise of deep learning. The main difference between this section and the last is the type of images that were worked with. For the task of medical image segmentation, there are many image modalities such as MRI, CT, X-ray and others. The challenge with medical images, however, there is a limited amount of readily available labeled data-sets. In order to use the techniques mentioned in the previous section, researchers would heavily depend on data augmentation, something that is still prominent in deep learning models.

% notable deep learning approaches
The rise of deep learning techniques in computer vision has been tremendous in the recent past and has been heavily used in medical image segmentation due to its ability to learn and extract features on its own, without the need of hand crafted features, priors or immensely large data-sets. The first to propose a fully convolutional architecture for semantic segmentation was \cite{long2015fully}. Medical image segmentation is a significant part of computer vision for many reasons. For one, having a robust and reliable method of detecting the presence of severity of a disease will positively impact clinical care. Medical image segmentation is often the first step in a diagnosis analysis plan. \cite{aggarwal2011role} explains that accurate segmentation is a key step in treatment planning.

Convolutional and pooling layers were used to learn the semantic and appearance information and produce pixel-wise prediction maps. This work enabled predictions on input images of arbitrary sizes. However, the predicted object boundaries often look blurred due to the reduction of the resolution after applying a series of convolutional and pooling layers. To mitigate the issue of reduced resolution, \cite{badrinarayanan2015segnet} proposed an encoder-decoder architecture that maps the learned low-resolution encoder feature maps to the original input resolution. Adding onto this encoder-decoder approach, \cite{yu2015multi} proposed an architecture that uses dilated convolutions to increase the receptive field in an efficient manner while aggregating multi-scale semantic information. \cite{ronneberger2015u} proposed adding skip connections at different resolutions. In recent years, many 2D and 3D deep learning architectures for segmentation have demonstrated promising results. 

%\cite{milletari2016v,oktay2018attention,hatamizadeh2018automatic}.

\section{Noteworthy Deep Learning Architectures}

In this section, the three architectures which were the main inspirations for the deep learning models developed in Chapter 3, 4 and 5 are discussed in more detail.

\subsection{UNet}

The UNet architecture, introduced by \cite{ronneberger2015u}, was one of the first convolutional networks designed specifically for bio medical imaging. This network aimed to tackle two issues that are specific to the domain in medical image segmentation. The first issue is the lack of large data-sets in this domain. The goal of this architecture is to produce competitive segmentation results, given a relatively small quantity of data. The lack of data availability is a huge drawback in medical image segmentation. Traditional feed-forward convolutional neural networks, with a fully connected layer at the end, have a large number of parameters to learn, hence require large data-sets. These models have the luxury of learning little bits of information over a vast number of examples and aggregate all that information into a generalized model. In the case of medical image segmentation, where there is a lack of data, the model needs to maximize the information learned from each example. Encoder-decoder architectures such as UNet have proven to be more effective even with small data-sets because the fully connected layer is replaced with a series of up convolutions on the decoder side, which still has learnable parameters, but much fewer than a fully connected layer. The second issue they tackle using this architecture is to accurately capture context and localize lesions at different scales and resolutions. The effectiveness of this simple and elegant architecture was one of the major inspirations for tackling the task of 2D medical image segmentation in this work.

\paragraph{Architecture Details}
\begin{figure}
  \includegraphics[width=\linewidth]{Images/og_unet.png}
  \caption{Original UNet Architecture from \cite{ronneberger2015u}}
  \label{fig:og_unet}
\end{figure}

The UNet architecture consists of two portions, as shown in Figure \ref{fig:og_unet}. The left side is a contracting path, in which successive convolutions are used to increase resolutions and learn features for lesion segmentation. The right side is an expanding path of a series of upsampling operations. To assist in lesion localization, low resolution features from the contracting path are combined with upsampled outputs from the expanding path. This is done via skip connections. This is significant to help gain spacial context that may have been lost while going through successive convolutions on the contracting path. 

An important aspect of this architecture is the upsampling path. This path utilizes a large number of feature channels which allows for effective propagation of context information to lower resolution layers on the contracting path, allowing for more precise localization. This thought process contributes to why the authors decided to make the expanding path symmetric to the contracting path, forming a "U" shaped architecture. 

The authors also mention another noteworthy issue faced for medical image segmentation, namely the problem of having objects of the same class touching each other with fused boundaries. To alleviated this issue, they propose using a weighted loss by separating background labels between touching segments to contribute to a large weight in the loss function.

\paragraph{Training}
The model is trained with input images and their corresponding segmentation maps via stochastic gradient descent. The authors utilize a pixel-wise softmax function over the final segmentation and combine it with a cross entropy loss function. The authors also make a special mention regarding weight initialization for the architecture before beginning training. Weight initialization is important to help control regions with excessive activation that over contribute to learning the correct weight parameters and ignoring other regions. They recommend initializing the weights for each feature maps so that the network has unit variance. To achieve this for the UNet architecture, the authors recommend drawing the initial weights from a Gaussian distribution. The authors also discussed the importance of data augmentation since medical image data-set are often so small. Techniques such as shifting, rotating, and adding noise are most popular for medical images.

The success of this architecture makes it very appealing to explore and build from for different medical segmentation tasks. The authors of the UNet paper demonstrated the success of this model on a cell segmentation task. We will take this architecture as a baseline for our task of lesion segmentation in the brain and lung in Chapter 4.

\subsection{DenseNet}

The DenseNet architecture was first introduced by \cite{DenseNet}. Although this architecture was not designed specifically for the application of medical image segmentation, the ideas can be effectively applied to the medical imaging domain. Before discussing the use case of the DenseNet in the medical domain, we first discuss the basics of the DenseNet architecture as discussed in \cite{DenseNet}.

\paragraph{Architecture Details}

\begin{figure}
  \includegraphics[width=\linewidth]{Images/og_dense.png}
  \caption[Original DenseNet Architecture from \cite{DenseNet}.]{Original DenseNet Architecture from \cite{DenseNet}. The top figure depcits an example dense block. The bottom figure depicts a full DenseNet architecture.}
  \label{fig:og_dense}
\end{figure}

DenseNet, depicted in Figure \ref{fig:og_dense}, is a network that connects each layer
to every other layer. This architecture extends on the observations that deep convolutional networks are highly accurate, and faster to train if there are shorter connections between input and output layers. Therefore, each layer takes the feature maps generated from all preceding layers and the current feature maps as input for all successive layers. Interestingly enough, there are actually fewer parameters to learn in this approach than others, such as ResNet, proposed by \cite{he2016deep}, because it does not learn redundant information. Instead, each layer takes what is already learned before as input, to prevent redundant learning. In addition to efficient parameter learning, the
back propagation of gradients are much smoother. Each layer has access to the gradients from the loss function and the original input signal, leading to an implicit deep supervision. This also contributes to natural regularization which is beneficial to for small data-set, where outfitting is often an issue. 

As mentioned previously, one goal of DenseNet is to improve information flow for fast and efficient back propagation. For comparison's sake, lets first consider how information flows through an architecture such as ResNet. In a traditional feed forward convolutional network, at each transition layer is described as $x_{l} = Z_{l}(x_{x-1})$. Z is a composite of convolution, batch norm, and ReLU operations. ResNet also has a residual connection to the previous layer. The composite function is the following:
\begin{equation}
\begin{split}
\label{eq:conv}
x_{l} = Z_{l}(x_{x-1}) + x_{l-1}
\end{split}
\end{equation}

Although the connection to the previous layer assists in gradient flow, the summation makes gradient flow somewhat slow. 

To combat this issue, the DenseNet uses concatenation instead of summation for information flow, as in the following, where $[a;b;c]$ denotes concatenation.
\begin{equation}
\begin{split}
\label{eq:conv}
x_{l} = Z_{l}([x_{l-1}; x_{l-2}; ...; x_{0}])
\end{split}
\end{equation}

This idea is referred to as dense connectivity. DenseNet is a collection of such dense blocks with intermediate convolution and pooling layers, as shown in Figure \ref{fig:og_dense}b.

The main points of success for this model is that it is a "lighter" model since there is not redundancy in learning parameters. Another point of success is that the concatenation of all prior feature maps makes gradient back propagation more efficient to assist in faster learning. In the remainder of this chapter, we explore how we can combine the UNet and DenseNet architecture to effectively and efficiently perform the task of lesion segmentation in the brain, and lung. Ideas from DenseNet have inspired the work in Chapters 3 and 4.

\subsection{VNet}

The VNet architecture was introduced by \cite{milletari2016v}. The structure of the VNet is very similar to that of the UNet, as seen in Figure \ref{fig:vnet}. The motivation for this architecture was that most medical image data is in 3D but most deep learning models at the time seemed to focus on 2D medical image segmentation models. Therefore, the authors developed an end-to-end 3D image segmentation framework, tailored for medical images. 

\paragraph{Architecture Details}

\begin{figure}
  \includegraphics[width=\linewidth]{Images/vnet.png}
  \caption{Original VNet Architecture from \cite{milletari2016v}.}
  \label{fig:vnet}
\end{figure}

The VNet architecture consists of a compression path on the left, which reduces resolution and an expansion path on the right, which brings the image back to the original dimensions, as shown in Figure \ref{fig:vnet}. On the compression path, convolutions are performed to extract image features, and at the end of each stage, reduce the image resolution before continuing to the next stage. On the decompression path the signal is decompressed and the original image dimensions are restored.

The main difference between the VNet and the UNet lies in the operations applied at each stage. In a classic UNet, as seen in Figure \ref{fig:og_unet}, at each stage, the compression path performs convolutions to extract features at a given resolution and then reduces the resolution before passing onto the next stage. In the case of the VNet, the compression path also performs convolutions at each resolution to extract features and the reduces the resolutions before passing onto the next stage. However, for the VNet, the input of each stage is used in the convolutional layers of that stage and is also added to the output of the last convolutional layer of that stage. This is done to enable the learning of a residual function, hence, residual connections are added in each stage. The authors observed that learning a residual function cuts the convergence times significantly. This is significant because the gradient can flow directly from the output of each stage to the input via residual connections during back propagation.

Another notable difference between the VNet and the UNet is the technique used to reduce resolutions between stages. In the case of the UNet, after an input goes through convolutions and a non linearity function, the input is fed into a max pool layer to reduce resolution. In the case of the VNet, the input is fed through a convolution with 2 $\times$ 2 $\times$ 2 voxels wide kernel applied with stride 2, after the non-linearity function. As a result, the feature maps are halved in size before proceeding to the next stage. According to the authors, this strategy is more memory efficient than a max pooling operation. Memory efficiency is highly advantageous since memory scarcity is a big problem for most 3D models. 

%The downsampling process on the compression side allows to compress the original signal size while increasing the receptive field via feature maps generated through the convolutions at different stages.

The expansion portion of the VNet extracts features and enables the spacial understanding from low resolution feature maps in order to build a final volumetric segmentation. After each stage of the expansion path a de-convolution operation is used to double the size of the input, until the original image dimensions are restored. The final feature maps are passed through a softmax layer to get a probability map predicting whether each voxel belongs to the background or foreground. Residual functions are also applied on the expansion path. 

The main point of success for this model is that it was the first end-to-end framework for 3D image segmentation in an effective and efficient manner. It utilized an encoder-decoder scheme with learned residual functions which allows in faster convergence times than other 3D networks. It employs convolutions for resolution reduction instead of using a max pooling layer, which is more memory efficient that and a very important point for 3D architectures. VNet and its variants have shown to be very promising in a variety of 3D segmentation tasks such as multi-organ abdominal segmentation, by \cite{gibson2018automatic}, and pulmonary lobe segmentation, by  \cite{imran2019automatic}. This architecture will be further explored in Chapter 5.
